Cover Tree Compressed Sensing for Fast MR Fingerprint Recovery

We adopt data structure in the form of cover trees and iteratively apply approximate nearest neighbour (ANN) searches for fast compressed sensing reconstruction of signals living on discrete smooth manifolds. Levering on the recent stability results for the inexact Iterative Projected Gradient (IPG) algorithm and by using the cover tree's ANN searches, we decrease the projection cost of the IPG algorithm to be logarithmically growing with data population for low dimensional smooth manifolds. We apply our results to quantitative MRI compressed sensing and in particular within the Magnetic Resonance Fingerprinting (MRF) framework. For a similar (or sometimes better) reconstruction accuracy, we report 2-3 orders of magnitude reduction in computations compared to the standard iterative method which uses brute-force searches.

==> cam_ready - arxiv2/sections/CSIPA.tex <==
\section{Iterative approximate projected Gradient}
\label{sec:CSIPA}


\subsection{Approximate projection} 
For saving computations, we consider each iteration of \eqref{eq:IPGD} calculates an approximate (inexact) projection step.
% For that we require to first define the set of $\varepsilon$-close projections of x onto $\Mm$ as follows:   
%\eq{
%\Pp_\Mm^{\epsilon}(x) := \{ z\in \Mm :\,	\norm{z-x}^2 \leq \inf_{z'\in \Mm} \norm{z'-x}^2 + \epsilon \}
%}.
%
%For a nonempty $\Mm$ Blumensath \nref showed that $\Pp_\Mm^{\epsilon}(.)$ is nonempty.
%Then, by $\pp_\Mm^{\epsilon}(x)$ we denote a point $p\in \Mm$ belonging to that set:
%\eq{
%\pp_\Mm^{\epsilon}(x) := p \in \Pp_\Mm^{\epsilon}(x).
%}
%
For that we first define the notion of $\epsilon$-close projection of x onto $\Mm$ 
\eql{\label{eq:eproj}
	\Pp_\Mm^{\epsilon}(x) \in \{ u\in \Mm :\,	\norm{u-x}^2 \leq \inf_{u'\in \Mm} \norm{u'-x}^2 + \epsilon \}.
}
Note that the point $\Pp_\Mm^{\epsilon}(x)$ may not be unique but for a nonempty $\Mm$ it exists (see \nref Blumensath also care must be taken when $\epsilon\rightarrow 0$). 

We update the algorithm \eqref{eq:IPGD} to the following \emph{inexact IPGD} version:
\eql{\label{eq:eIPGD}
	x^{t+1} = \Pp_\Mm^{\epsilon_{t}} \left( x^{t} - \mu A^*(Ax^{t}-y) \right). 
}
where $\epsilon_t$ denotes the level of approximation for calculating  the projection step at iteration $t$.


\subsection{Convergence result}
Assume $A$ satisfies Bi-Lipschitz property with respect to $\Mm$ with constants $\alpha,\beta$ defined as follows. 


\marginpar{we don't need universal $\alpha$..just $\alpha_{x_0}$. Not same argument for $\beta$ tho}
{\thm Assume $A$ is Bi-Lipschitz w.r.t. $\Mm$ with constants satisfying $\beta < 1.5\alpha$. For the step size $\mu$ chosen so that $2/3\alpha^{-1}<\mu\leq\beta^{-1}$, the sequence generated by Algorithm \eqref{eq:eIPGD} obeys the following bound:
	%generates a sequence the solution of $\epsilon$-IPGD after $t$ iterations satisfies:
	\begin{align}
&\norm{x^{t}-x_0}^2 \nonumber \\
&\leq \rho^t  \left( \norm{x^{init}-x_0}^2 +   \frac{2}{\mu\alpha}\sum_{i=0}^{i=t} \rho^{-i} \epsilon_i \right) + \frac{4(1-\rho^t)}{\alpha(1-\rho)}\norm{w}^2. 
\end{align}
Where $\rho= 2\left(\frac{1}{\mu\alpha}-1 \right)$, and $e$ denotes the noise in the forward model  i.e. $w=y-Ax_0$.
	}

\begin{proof}
Set $g = 2A^*(Ax^t-y)$ i.e. the gradient of $\norm{y-Ax^{t}}^2$. Then we have	
\begin{align*} 
	&\norm{y-Ax^{t+1}}^2-\norm{y-Ax^{t}}^2	\\
	&= \langle x^{t+1}-x^t,g \rangle +\norm{A(x^{t+1}-x^t)}^2 \\
	&\leq \langle x^{t+1}-x^t,g \rangle + \beta \norm{x^{t+1}-x^t}^2, 
\end{align*}
where the last inequality follows from the Bi-Lipschitz property \eqref{eq:bilip} of $A$. Assuming $\beta \leq 1/\mu$, we have
\begin{align*}
&\langle x^{t+1}-x^t,g \rangle + \beta \norm{x^{t+1}-x^t}^2 \\
 & \leq \langle x^{t+1}-x^t,g \rangle + \frac{1}{\mu} \norm{x^{t+1}-x^t}^2\\
& = \frac{1}{\mu} \norm{x^{t+1}-x^t+\frac{\mu}{2} g }^2 - \frac{\mu}{4} \norm{g}^2 .
\end{align*}
Because of \eqref{eq:eIPGD}, \eqref{eq:eproj} and the fact that $x_0\in\Mm$ we have
\eq{
	\norm{x^{t+1}-x^t+\frac{\mu}{2} g }^2 \leq  \norm{x_0-x^t+\frac{\mu}{2} g }^2 +\epsilon_t.	
}
Therefore we can write
\begin{align}
&\norm{y-Ax^{t+1}}^2-\norm{y-Ax^{t}}^2 \nonumber	\\
%&=\langle x^{t+1}-x^t,g \rangle + \frac{1}{\mu} \norm{x^{t+1}-x^t}^2 \nonumber\\
&\leq \frac{1}{\mu} \norm{x_0-x^t+\frac{\mu}{2} g }^2 - \frac{\mu}{4} \norm{g}^2 +\frac{\epsilon_t}{\mu} \nonumber \\
&= \langle x_0-x^t,g \rangle + \frac{1}{\mu} \norm{x_0-x^t}^2 +\frac{\epsilon_t}{\mu} \label{eq:p1b2}
\end{align}



Similarly we can use the lower Bi-Lipschitz constant to obtain an upper bound on $ \langle x_0-x^t,g \rangle$:
\begin{align*} 
\norm{ \underbrace{y-Ax_0}_{w}}^2-\norm{y-Ax^{t}}^2	&= \langle x_0-x^t,g \rangle +\norm{A(x_0-x^t)}^2 \\
&\geq \langle x_0-x^t,g \rangle + \alpha \norm{x_0-x^t}^2.
\end{align*}
Using this bound in \eqref{eq:p1b2} and cancelling $-\norm{y-Ax^t}^2$ from both sides of the inequality, we can deduce
\begin{align*}
&\norm{y-Ax^{t+1}}^2 \leq \left(\frac{1}{\mu}-\alpha \right)\norm{x^t-x_0}^2 + \norm{w}^2+ \frac{\epsilon_t}{\mu}.
\end{align*}
Finally we use again the lower Bi-Lipschitz constant to lower bound  $\norm{y-Ax^{t+1}}^2$:
\begin{align*}
&\alpha\norm{x^{t+1}-x_0}^2\leq \norm{A(x^{t+1}-x_0)}^2 \\
&=\norm{Ax^{t+1}-y+w}^2
\leq 2 \norm{Ax^{t+1}-y}^2+ 2\norm{w}^2.
%\norm{y-Ax^{t+1}}^2 &\leq \norm{A(x_0-x^{t+1})+Aw}^2\\
%&\leq 2\norm{A(x_0-x^{t+1})}^2+ 2\norm{Aw}^2
%&\Longrightarrow \norm{y-Ax^{t+1}}^2 \geq 
\end{align*}
The last inequality uses the triangle inequality and the fact that $(a+b)^2\leq 2a^2+2b^2$. 
As a result, we can deduce the following bound for noisy case:
\begin{align}\label{eq:iterbound}
	\norm{x^{t+1}-x_0}^2 \leq 2\left(\frac{1}{\mu\alpha}-1 \right)\norm{x^t-x_0}^2 + \frac{4}{\alpha}\norm{w}^2+ \frac{2}{\mu\alpha}\epsilon_t,
\end{align}

\todo{Note that for noiseless case $y=Ax_0$ it holds that:
\eq{
	\norm{y-Ax^{t+1}}^2= \norm{A(x^{t+1}-x_0)}^2 \geq \alpha\norm{x^{t+1}-x_0}^2,
}
and therefore we can get sharper bound here:
\begin{align}\label{eq:boundnoiseless}
\norm{x^{t+1}-x_0}^2 \leq \left(\frac{1}{\mu\alpha}-1 \right)\norm{x^t-x_0}^2 +  \frac{1}{\mu\alpha}\epsilon_t,
\end{align}}

We apply the previous bound recursively and complete the proof:
\begin{align}
&\norm{x^{t}-x_0}^2 \nonumber \\
&\leq \rho^t  \norm{x^{init}-x_0}^2 +  \frac{4}{\alpha}\norm{w}^2 \sum_{i=0}^{i=t} \rho^i+ \frac{2}{\mu\alpha}\sum_{i=0}^{i=t} \rho^{t-i} \epsilon_i
\end{align}
for $\rho= 2\left(\frac{1}{\mu\alpha}-1 \right)$. Note that for convergence we require $\rho<1$ and therefore a lower bound on the step size which is $1/\mu< 3\alpha/2$.
\end{proof}


{\rem{We achieve a linear convergence (to a solution within $\frac{4(1-\rho^t)}{\alpha(1-\rho)}\norm{w}^2$ distance from $x^0$) as long as $\epsilon_t$ linearly decays to zero:
	\eq{ \norm{x^{t}-x_0}^2 \leq \frac{4(1-\rho^t)}{\alpha(1-\rho)}\norm{e}^2+o( r^t) 
	}	
	\marginpar{shall we say convergence or error decay??} 
	For $\epsilon_t=o(\rho^t)$ we can establish a rate convergence $r=\rho$ similar as for the IPGD algorithm \eqref{eq:IPGD} with the exact projection (see Theorem.2 \cite{Blumen}). 
An approximation with a slower rate of decay, i.e. $\epsilon_t=\Theta(\bar{\rho}^t)$ where $\bar{\rho}<\rho$, decreases the convergence rate of \eqref{eq:eIPGD} to $r=\bar{\rho}$.	
%If decays with a slower rate $\rho'<\rho$, then the rate of convergence of \eqref{eq:eIPGD} will be  
Finally for $\epsilon_t=\Theta(\rho^t)$, we have $r=\rho+ \delta$ for an arbitrary small $\delta>0$.	 	
	}}
	
	
\subsection{Adaptive approximation level}
\todo{Not sure if this part will be useful...didn't work well for MRF simulations}
If we don't know how to set $\epsilon_t$ to decay (probably since we don't know $\rho$), we can for instance do the following adaptive procedure:
\subsubsection{Objective Feedback}
For some constant $0<\gamma<1$ we set the approximation level proportional to the current objective function value:
\eql{\label{eq:adaptive-e}
	\epsilon_t := \gamma \mu  \norm{y-Ax^t}^2.
	}	
% we consider each iteration of \eqref{eq:IPGD} calculates an approximate (inexact) projection step  which obeys the following bound: for solution at each iteration $x^t$ we have
%\eq{
%	\norm{x^t-\Pp_\Mm^\epsilon(x^t)}^2 \leq \norm{x^t-\Pp_\Mm(x^t)}^2 + \epsilon\norm{y-Ax^t}^2
%}	
%We note that the precision of the approximation is not fixed and gradually improved as the objective of \eqref{eq:opt1} decays.
%
%Assume $A$ satisfies Bi-Lipschitz property with respect to $\Mm$ with constants $\alpha,\beta$ defined as follows. 
%
%{\defn{ $A$ is Bi-Lipschitz w.r.t. $\Mm$, if $\forall x1,x2\in \Mm$ there exists constants $0<\alpha\leq \beta$ such that
%	\eql{
%		\alpha \norm{x1+x2}^2 \leq \norm{A(x1+x2)}^2\leq \beta \norm{x1+x2}^2  }	
%}}
The following theorem considers noiseless measurements \marginpar{and it can be extended to noisy measurements case probably with doubling the convergence rate} and states the IPGD convergence using the approximate projection scheme defined above.

{\thm{Assume $y=Ax_0$, and $A$ is Bi-Lipschitz w.r.t. $\Mm$ with constants satisfying $\beta\leq 2\alpha$. Set $0<\gamma<1$ and the step size $\mu>0$ such that
	$\beta \leq 1/\mu \leq (2-\gamma)\alpha$. The sequence generated by Algorithm \eqref{eq:eIPGD} obeys the following bound
	\eql{
		\norm{x^{t}-x_0}^2\leq 
		\left( \frac{1}{\mu\alpha}+\gamma-1\right)^t\norm{x^{init}-x_0}^2.		
	}
}}
\begin{proof}
	Continue from \eqref{eq:boundnoiseless} by substituting $\epsilon_t$ with \eqref{eq:adaptive-e} and then use $\alpha^{-1} \norm{y-Ax^t}^2\leq \norm{x^t-x_0}^2$ 
\end{proof}

\subsubsection{Gradient Feedback}
Norm of the gradient at each iteration can be used for tuning the approximation level i.e. for a positive constant $\gamma$:
\eql{\label{eq:adaptive-e2}
	\epsilon_t := \gamma \norm{g^t}^2 = \gamma\norm{A^*Ax^t-A^*y}^2.
}
	
{\thm{\label{thm:gradconv} Assume $A$ is bi-Lipschitz w.r.t. $\Mm$ with constants $\beta \leq \frac{3\alpha}{2(1+2\gamma\norm{A}^4)}$. Set the step size such that $\frac{2}{3}(1+2\gamma\norm{A}^4)\alpha^{-1}\leq \mu \leq\beta^{-1}$. The sequence generated by Algorithm \eqref{eq:eIPGD} using approximation \eqref{eq:adaptive-e2} obeys the following bound:
			\eql{
			\norm{x^{t}-x_0}^2 
			\leq \rho^t  \norm{x^{init}-x_0}^2  + \frac{4(1-\rho^t)}{\alpha(1-\rho)}\left(1+\gamma \frac{\norm{A}^2}{\mu}\right)\norm{w}^2,
		}
			where, $\rho= 2\left(\frac{1+2\gamma \norm{A}^4}{\mu\alpha}-1 \right)$, 
%\begin{align*}
%&\rho= 2\left(\frac{1+2\gamma \norm{A}^4}{\mu\alpha}-1 \right),\quad\eta=\frac{4(1-\rho^t)}{\alpha(1-\rho)}\left(1+\gamma \frac{\norm{A}^2}{\mu}\right),
%\end{align*}
				 and $w=y-Ax_0$ is the noise.
		}
	}
\begin{proof}
	We have that 
	\begin{align*}
	\gamma\norm{g^t}^2 &= \gamma\norm{A^*A(x^t-x_0)-A^*w}^2\\
	&\leq 2\gamma\norm{A^*A (x^t-x_0)}^2+2\gamma\norm{A^*w}^2\\
	&\leq 2\gamma\norm{A}^4\norm{x^t-x_0}^2+2\gamma\norm{A}^2\norm{w}^2.
	\end{align*}
\marginpar{not sure sharp enough!}The first inequality follows from $(a-b)^2\leq 2a^2+2b^2$. Applying this bound in \eqref{eq:iterbound} we achieve
\begin{align}\label{eq:iterbound2}
\norm{x^{t+1}-x_0}^2 \leq& 2\left(\frac{1+2\gamma \norm{A}^4}{\mu\alpha}-1 \right)\norm{x^t-x_0}^2 \nonumber \\ &+\frac{4}{\alpha}\left(1+\frac{\gamma}{\mu} \norm{A}^2\right)\norm{w}^2.
\end{align}
Applying recursively this bound competes the proof. Note that for convergence we require $\rho<1$ which implies the lower bound on $\mu$.
\end{proof}	

==> cam_ready - arxiv2/sections/conclusion.tex <==
\section{Conclusions}
We proposed an inexact IPG algorithm for data driven CS problem with an application to fast MRF parameter estimation. The projection step is implemented approximately by  using cover trees ANN searches.  Thanks to the IPG's robustness against approximations, by using this algorithm one achieves a  comparable (and sometimes empirically enhanced) solution precision to the exact algorithm  however with significantly less amount of  computations regarding iteratively searching through large datasets.% with low intrinsic dimensions.

==> cam_ready - arxiv2/sections/covertree.tex <==
\section{Cover tree for fast nearest neighbour search}

With the data driven CS formalism and discretization of the model  %$\Cc = \prod_{i=1}^N \Mb$, 
the projection step of IPG reduces to a search for the nearest atom in each of the product spaces, however in a potentially very large $d$ size dictionary. %Therefore the linear complexity of an exact projection in $d$ can still be a bottneck  an extract IPG %which brings a serious bottleneck to searches with a linear complexity in term of $d$.  
Thus search strategies with linear complexity in $d$, e.g. an exhaustive search, can be a serious bottleneck for solving such problems. %We address this issue by replacing the exhaustive search with fast approximate searches. 
A very well-established approach to overcome the complexity of an exhaustive NN search on a large dataset 
consists of hierarchically partitioning the solution space and forming a \emph{tree} structure whose nodes representing those partitions, and then using a  branch-and-bound method on the resulting tree for a fast Approximate NN (ANN) search with $o(d)$ complexity. 
In this regard, we address the computational shortcoming of the projection step in the exact IPG by preprocessing $\widetilde \Cc$ and form a \emph{cover tree} structure suitable for fast ANN searches \cite{beygelzimer2006cover,Navigating}. 


A cover tree is a levelled tree whose nodes (i.e. associated data points) at different scales form covering nets for data points at multiple resolutions. Denote by $\Ss_l$ the set of nodes appearing at scale $l=1,\ldots,L_{\max}$ and by $\sigma:=\max_{\psi\in\widetilde \Cc}\norm{\psi_\text{root}-\psi}$ the maximal coverage by the root, then a cover tree structure must have the following  three properties:
\begin{enumerate}
	\item Nesting: $\Ss_l \subseteq \Ss_{l+1}$, once a point $p$ appears as a node in $\Ss_l$, then every lower level in the tree has that node.
	\item Covering: every node $q\in \Ss_{l+1}$ has a parent node  $p\in \Ss_{l}$, where $\norm{p-q}\leq \sigma2^{-l} $. As a result, covering becomes finer at higher scales in a dyadic fashion. 
	%and For every $p\in \Ss_{i−1}$, there exists
	%a q 2 Ci such that d(p, q) < 2i and the node in
	%level i associated with q is a parent of the node
	%in level i − 1 associated with p.
	
	\item Separation: nodes belonging to the same scale are separated by a minimal distance which dyadically shrinks at higher scales i.e. $\forall q,q'\in\Ss_l$ we have $\norm{q-q'}>\sigma2^{-l}$.   
\end{enumerate}  
Each node $p$ also keeps the maximum distance to its descendants denoted by
$\mathrm{maxdist}(q):= \max_{q'\in \text{descendant}(q)} \norm{q-q'}\leq \sigma2^{-l+1}$. 
which will be useful for fast NN/ANN search.\footnote{Note that any node $q\in \Ss_l$ due to the covering property satisfies 
$maxdist(q) \leq \sigma \left( 2^{-l}+2^{-l-1}	+ 2^{-l-2}+\dots \right)
< \sigma 2^{-l+1}$ and thus, one might avoid saving $maxdist$ values and use this upper bound instead.}
The \emph{explicit} tree representation requires the storage space $O(d)$~\cite{beygelzimer2006cover}. 


\begin{algorithm}[t]
	\label{alg:findNN}
	\SetAlgoLined
	$Q_0 = \{\Ss_0\}$, $\Ss_0$ the root of $\Tt$, 
	%\If{$q_c=\{\}$}{$q_c=\Ss_0$}  
	$\d_{\min}=\norm{p-q_c}$\\
	$l=0$\\
	\While{$l<L_{\max}$ \, \text{AND} \, $\sigma 2^{-l+1}(1+\epsilon^{-1})> \d_{\min}$\,}
	{
		$Q=\left\{\text{children}(q):\, q\in Q_l \right\} $\\
		$q^* = \argmin_{q\in Q} \norm{p-q}$, \quad $\d = \norm{p-q^*}$ \\
		\If{$\d<\d_{\min}$}{$\d_{\min}=\d, \quad q_c=q^*$}
		$Q_{l+1} = \left\{q\in Q: \norm{p-q}\leq \d_{\min} + \mathrm{maxdist}(q) \right\}$\\
		$l  = l+1$\\
	}	
	\Return $q_c$\\%=\argmin_{q\in Q_{L_{\max}}} \norm{p-q}$\;
	\caption{\label{alg:NN} \textbf{$(1+\epsilon)$-ANN}(cover tree $\Tt$, query point $p$, current estimate $q_c \in \widetilde \Cc$),\quad  accuracy parameter $\epsilon$}
\end{algorithm}

{\defn{\label{def:eNN}Given a query $p$, 
		%which might not belong to $\widetilde \Cc$ 
		$q\in\widetilde \Cc$ is a $(1+\epsilon)$-ANN of $p$ for an $\epsilon\geq 0$ if it holds:
		$\norm{p-q} \leq (1+\epsilon)\inf_{u\in\widetilde \Cc}\norm{p-u}.$
			}}	
\newline
			
Algorithm \ref{alg:NN} details the branch-and-bound procedure for $(1+\epsilon)$-ANN search on a given cover tree (proof of correctness is available  in~\cite{beygelzimer2006cover}).
In short, we iteratively traverse down the cover tree and at each scale we populate the set of \emph{candidates} $Q_l$ with nodes which could be the ancestors of the solution and discard others (this refinement uses the triangular inequality and the lower bound on the distance of the grandchildren of $Q$ to $p$, based on  $\mathrm{maxdist}(q)$).  At the finest scale (before stopping) we search the whole set of final candidates and report an $(1+\epsilon)$-ANN point. Note that at each scale we only compute distances for non self-parent nodes (we pass, without computation, distance information of the self-parent children to finer scales). 
The case $\epsilon=0$ refers to the exact tree NN search where one has to continue  Algorithm~\ref{alg:NN} until the finest level of the tree.   One should distinguish between this strategy and performing a brute-force search. Although they both perform an exact NN search, the complexity of Algorithm~\ref{alg:NN} 
%the proposed algorithm in~\cite{beygelzimer2006cover} 
is empirically shown to be way less in practical datasets.


Although the cover tree construction is blind to the explicit structure of data, several key growth properties such as the tree's explicit depth, the number of children per node, and importantly the overall search complexity are characterized by the intrinsic \emph{doubling dimension} of the model~\cite{Navigating}. 
Practical datasets are often assumed to have small doubling dimensions e.g. when $\widetilde \Cc \subseteq \Mm$  %uniformly
samples a $K$-dimensional manifold $\Mm$ with certain  regularity, one has $\dim_D(\widetilde \Cc)\leq \dim_D(\Mm)=O(K)$ \cite{dasgupta2008}. 
The following theorem bounds the complexity of  $(1+\epsilon)$-ANN cover tree search~\cite{Navigating,beygelzimer2006cover}: 
		{\thm{\label{thm:NNcomp2}Given a query which might not belong to $\widetilde \Cc$, the approximate $(1+\epsilon)$-ANN search on a cover tree takes at most 
				\eql{
					2^{O(\dim_D(\widetilde \Cc))}\log \Delta+(1/\epsilon)^{O(\dim_D(\widetilde \Cc))} 
				}
				computations in time with $O(\#\widetilde \Cc)$ memory requirement, where  $\Delta$ is the aspect ratio\footnote{The aspect ratio of a set $\Cc$ is $\Delta:=\frac{\max \norm{q-q'}}{\min \norm{q-q'}}$, $\forall q\neq q'\in \Cc$.} of $\widetilde \Cc$  and $\#$ stands for set cardinality.}	
		}
		
		For most applications $\log (\Delta) = O(\log(d))$~\cite{Navigating} and thus for datasets with low dimensional structures i.e. $\dim_D=O(1)$ and by using  moderate approximations one achieves a search complexity logarithmic in $d$, as opposed to the linear complexity of a brute-force search.
		
		Note that the complexity of an \emph{exact} cover tree search could be arbitrary high i.e. linear in $d$, at least in theory (unless the query belongs to the dataset~\cite{beygelzimer2006cover} which does not generally apply e.g. for the intermediate steps of the IPG). %And thus the same applies to the FP and PFP type ANN searches since they are also based on performing exact NN (on a truncated tree). 
		However in our experiments we empirically observe  that the complexity of an exact cover tree NN is still much lower than performing an exhaustive search.


\subsection{Inexact data driven IPG algorithm}
%\section{Iterative Projection Accelerated with Cover Tree Search}
We use cover tree's $(1+\epsilon)$-ANN approximate search to efficiently implement the cone projection step of the data driven IPG algorithm. %We first normalize the atoms $\psi_i$ and build a cover tree structure $\Tt$ for this dictionary.
We only replace the exact search step \eqref{eq:exactP} with the following approximation:
\eql{\label{eq:ANN1}
	\psi_{i^*} = \textbf{$(1+\epsilon)$-ANN}\left( \Tt,\frac{Z_j}{\norm{Z_j}}, \frac{X_j^k}{\gamma_j}\right), \quad \forall j=1,\ldots,J.
}
%Note that the dictionary $\Psi$ is normalized here. 
We denote by $\Tt$ the cover tree structure built for the normalized dictionary with atoms $\psi_i/\norm{\psi_i}$. For the current estimate we use the atom previously selected i.e. $X_j^k/\gamma_j$ for all $j$. We additionally normalize the gradient update $Z_j$ for the search input. This step may sound redundant however since all dictionary atoms are normalized and live on the  hypersphere, we empirically observed that this trick leads to a better  acceleration.

As a result by this update we obtain a $(1+\epsilon)$-approximate cone projection denoted by $\Pp^\epsilon_{\text{cone}(\widetilde \Cc)}(Z_j)$ satisfying definition \eqref{eq:eproj}. Therefore supported with an embedding assumption w.r.t. to the product model \eqref{eq:prod} and according to Theorem~\ref{th:inexactLS2} we can guarantee stable CS recovery using this algorithm with a small computational effort.
%
%{\thm{Fix a constant $\theta\in (0, 1/2]$ for which $A$ is bi-Lipschitz w.r.t. $\Mb$ with constants satisfying $\beta\leq \frac{3\alpha}{2(1+\theta)}$.		
%		 Let  $\epsilon=\frac{\theta}{6\mu^2\norm{A}^4}$, and set the step size such that $\frac{2}{3}(1+\theta)\alpha^{-1}\leq \mu \leq\beta^{-1}$. For $x^{init}=\Ss_0$, the sequence generated by Algorithm \eqref{eq:IPACTS} obeys the following bound:
%					\eql{
%						\norm{x^{t}-x_0}^2 
%						\leq \rho^t  \sigma^2  + \frac{4(1-\rho^t)}{\alpha(1-\rho)}\left(1+ \frac{\theta}{2\mu\norm{A}^2}\right)\norm{w}^2,
%					}
%					where $\rho = 2\left(\frac{1+\theta}{\mu\alpha}-1\right)$ and $\sigma=\max_{q\in\Mb}\norm{\Ss_0-q}$.  The ANN cost per iteration is at most 
%					\eq{
%						2^{O(\dim(\Mb))}\log \Delta+(\mu \norm{A}^2/\sqrt{\theta})^{O(\dim(\Mb)).} 
%					}
%		}
%	}
%\begin{proof}
%According to Definition \ref{def:eNN}, the updates of \eqref{eq:IPACTS} follow the bound below:
%\begin{align*}
%\norm{x^{t+1}-x^t+\mu g^t}^2 &\leq (1+\epsilon)^2 \inf_{x\in\Mb}\norm{x-x^t+\mu g^t}^2 \\
%&\leq (1+3\epsilon) \inf_{x\in\Mb}\norm{x-x^t+\mu g^t}^2 \\
%&\leq \norm{x_0-x^t+\mu g^t}^2 + 3\epsilon\mu^2\norm{g^t}^2\\
%\end{align*}	
%The second inequality follows from $(1+\epsilon)^2\leq1+3\epsilon$ for $e\in[0,1]$. Substituting $x$ partly with $x_0$ and $x_t$ (both in $\Mb$) results the last inequality. 
%
%As a result $(1+\epsilon)$-ANN search provides an inexact projection step with \emph{gradient feedback} similar to \eqref{eq:adaptive-e2}. Set \eq{\gamma = 3e\mu^2=\frac{\theta}{2\norm{A}^4}
%	} 
%	in Theorem \ref{thm:gradconv} and the convergence bound follows. Using Theorem \ref{thm:NNcomp2} for    $e=\frac{\theta}{6\mu^2\norm{A}^4}$ bounds the computational cost of the approximate NN per iteration.
%\end{proof}


==> cam_ready - arxiv2/sections/datadrivenCS.tex <==
\section{Data driven CS in product space}
\label{sec:datadrivenCS}
%Many CS reconstruction programs resort to signal models promoted by certain (semi) algebraic functions $h(x):\RR^n\rightarrow \RR_+\cup\{ 0\}$. For example we can have \marginpar{\red{Start BETTER this part..if mike can rewrite}}
%\eq{\Cc := \big\{x\in \RR^n : h(x)\leq \zeta\big\},
%	}
%where $h(x)$ may be chosen as the $\ell_{0}$ or $\ell_{0-2}$ semi-norms or as the $\rank(x)$  which promotes sparse, group-sparse or low-rank (for matrix spaces) solutions, respectively. One might also replace those penalties with their corresponding  %algebraic and 
%convex relaxations namely, the $\ell_1$, $\ell_{1-2}$ norms or the nuclear norm. 

Data driven CS corresponds to cases where in the absence of an algebraic (semi-algebraic) physical model one resorts to collecting a large number of data samples in a dictionary and use it e.g. as a \emph{point cloud} model for CS reconstruction~\cite{RichCSreview}.  
%In this case the model is $\Cc = \bigcup_{i=1}^{d}\{\psi_i\}$ where $\psi_i\in\RR^n$s are atoms of a $n\times d$ dictionary $\Psi$. %\{\psi_i\}_{i=1}^{d}$
% of $d$ points (atoms) in $\RR^n$ the model becomes.  
Data driven CS finds numerous applications e.g. in hyperspectral imaging (HSI)~\cite{TIPHSI}, mass spectroscopy (e.g. MALDI imaging) \cite{Kobarg2014} and MRF recovery~\cite{MRF,BLIPsiam} just to name a few. For instance the USGS Hyperspectral library\footnote{\url{http://speclab.cr.usgs.gov}} contains the spectral signatures of thousands of substances. This side-information is shown to enhance CS recovery and classification~\cite{TIPHSI,meEUSIPCO10}. Here the model is discrete and nonconvex:
\eql{\label{eq:dmodel}
	\widetilde \Cc:=\bigcup_{i=1}^{d}\{\psi_i\} \in \CC^{\n}}
and it corresponds to atoms of a (possibly complex-valued) dictionary $\Psi$ customized for e.g. HSI, MALDI or MRF data.



%Recently MR Fingerprinting~\cite{MRF} proposed a fast CS acquisition scheme for quantifying the NMR properties (such as the $T1,T2$ relaxation times, off-resonance frequencies, proton density) of tissues. Since random excitation sequences generate magnetization responses in non-analytic forms, \cite{MRF} proposed build a very large dictionary of fingerprints driven by the Bloch dynamic equations for all combination of those parameters. 


%the set $\Cc$ may also be a dense collection of samples from a continuous algebraic manifold with a non trivial projection e.g. Magnetic resonance fingerprinting \nref. 
% As the projection step might not be trivial or computationally easy for many complex manifolds we consider a data driven approach which consists of collecting discrete samples of the manifold in a dictionary and approximate 


 

%Recently MR Fingerprinting \cite{MRF} proposed a fast CS acquisition scheme for quantifying the NMR properties (namely the $T1,T2$ relaxation times) of tissues. Small number of  excitations in form of rotating the magnetic field applies to the tissue, and between each two excitations, the \emph{partial} k-space information is measured. An iterative exact projection algorithm (BLIP) is proposed for the MRF problem which achieves a great parameter estimation accuracy \cite{BLIPsiam}. % versus compression trade-off $\nref$.
%The projection consists of NN searches on a densely sampled manifold $\Mb$ of fingerprints driven by the Bloch dynamic equations.

%\subsection{Data driven CS in product space}
A multichannel image such as HSI, MALDI or MRF can be represented by a $\n\times J$ matrix $X$, where $n=\n J$ is the total number of pixels, $J$ is the spatial resolution and $\n$ is the number of channels. 
%e.g. the spectral bands for an HSI.
%e.g. $\n=3$ for an RGB image or $\n\approx 400$ spectral bands for an HSI acquired by NASA's AVIRIS spectrometer.
% $\n\approx 5000$ for a MALDI image~\cite{Kobarg2014}.
 %In the simplest form 
%this matrix is a column sub-selection (with possible repetitions) of the dictionary 
%When the acquisition resolution is high enough so that the spectral contents do not merge spatially, one has
Under the \emph{pixel purity} assumption each spatial pixel corresponds to a certain material with specific signature. Considering a notion of \emph{signal intensity} in this model (e.g. due to variable illumination conditions in HSI, or a non-uniform proton density in MRF), the columns of $X$ belong to the \emph{cone} associated with the signatures~\eqref{eq:dmodel}. Denoting by $X_j$ the $j$th column of $X$ (i.e. a multi-dimensional spatial pixel), we have 
\eql{\label{eq:immodel}
	X_{j}\in  \text{cone}(\widetilde \Cc), \quad \forall j=1,\ldots,J,
} 
where the cone is also a discrete set defined as
\eq{
	\text{cone}(\widetilde \Cc):=\{x\in \CC^{\n}: x/\gamma \in \widetilde \Cc \,  \text{for some} \, \gamma>0 \}.
}	
Here, $\gamma$ corresponds to the signal intensity (per spatial pixel).


The CS sampling and reconstruction follows \eqref{eq:CSsampling} and \eqref{eq:opt1} by setting $x^*:=X_\text{vec}$ (by $X_\text{vec}$ we denote the vector-rearranged form of the matrix $X$) and the only update is that now  
%The CS reconstruction reads
%\eql{\label{eq:datadrivenCS}
%	\min_{\substack{X_j\in \text{cone}(\widetilde\Cc),\\ \forall j=1,...,J}} \big\{f(x):= \frac{1}{2}\norm{y-AX_\text{vec}}^2\big\}.
%}
%or equivalently and similar to problem \eqref{eq:p1} 
%\eq{
%	\min_{x\in \prod_{j=1}^J \text{cone}(\widetilde\Cc)} \big\{f(x):= \frac{1}{2}\norm{y-Ax}^2\big\}.
%}
%The only update w.r.t. problem \eqref{eq:p1} 
%is the fact that now 
the solution lives in a \emph{product space} of the same model i.e. 
\eql{
	\label{eq:prod}\Cc:=\prod_{j=1}^J \text{cone}(\widetilde\Cc)
} 

In a single dimensional setting i.e. $\Cc=\text{cone}(\widetilde \Cc)$,  
%and when the model is discrete discrete model $\Mm=\Mb$
  there will be no need for an IPG algorithm to solve problem \eqref{eq:opt1}. If the embedding holds with a $\mmx>0$ (i.e. an identifiability condition) then the atom with a maximum coherence $\langle A \psi_i/\norm{A \psi_i},y\rangle$ with the measurements identifies the correct signature in a \emph{single} iteration. 
However such a direct approach in a multi-dimensional setting $J\gg1$ 
 (e.g. when the sampling model non-trivially combines columns of $X$) generally has an \emph{exponential} $O(d^J)$ complexity because of the combinatorial nature of the product space constraints. A tractable scheme which has been frequently considered for this case e.g. in \cite{BLIPsiam} would be an IPG type algorithm~\eqref{eq:IPGD}.
 
 After the gradient update $Z_{\text{vec}}$ = $X_{\text{vec}}^k + \mu A^H(y-AX_{\text{vec}}^k)$, the projection onto the product model \eqref{eq:prod} decouples into separate cone projections for each spatial pixel $j$. The cone projection $\Pp_{\text{cone}(\widetilde \Cc)}(Z_j)$ follows the steps below: 
 \begin{align}\label{eq:exactP}
 &i^* = \argmin_i \norm{Z_j -\psi_i/\norm{\psi_i}} &\text{(NN search)}\\
 &X^{k+1}_j = \Pp_{\text{cone}(\widetilde \Cc)}(Z_j) = \gamma_j \psi_{i^*}& \text{(rescaling)}
 \end{align}
 where,  $\gamma_j = \max\left( \text{real}(\langle Z_j ,\psi_{i^*}\rangle)/  {\norm{\psi_{i^*}}^2},0\right)$ is the per-pixel signal intensity.
 
% i) a nearest neighbour (NN) search for the best match between the current gradient update $Z_j^{k}$ and  the normalized atoms of $\widetilde \Cc$ and ii) a rescaling step to get the current intensity estimate per pixel and update the solution $X^{k+1}$.% as $X_j^k = \gamma_jZ_j^k$. %rescale as follows/
 
% \begin{algorithm}[t]
% 	\SetAlgoLined
% 	$k=0, X^0=\mathbf{0}$\\
% 	\While{convergence}
% 	{ $Z_{\text{vec}}$ = $X_{\text{vec}}^k + \mu A^H(y-AX_{\text{vec}}^k)$\\
% 		\For{j=1,\ldots,J}{
% 		$i^* = \argmin_i \norm{Z_j -\frac{\Psi_i}{\norm{\Psi_i}}}$\\
% 		$\gamma_j = \max\left( \frac{\langle Z_j ,\Psi_{i^*}\rangle}  {\norm{\Psi_{i^*}}},0\right)$\\
% 		$X^{k+1}_j = \rho_j \Psi_{i^*}$
% 	}
% 		$k  = k+1$\\
% 	}	
% 	%\Return $q_c$\\%=\argmin_{q\in Q_{L_{\max}}} \norm{p-q}$\;
% 	\caption{Exact data driven IPG  	\label{alg:BLIP}}
% \end{algorithm}
 %Assume atoms of $\Psi$ are all normalized (and if not we perform such a preprocessing). 
 
% The projection of a point $z$ onto the cone($\psi_i$) associated with a single atom is:
% \eq{
% 	\Pp_{\text{cone}(\psi_i)}(z)= \max\left( \frac{\langle z , \psi_i \rangle}{\norm{\psi_i}^2},0\right) \psi_i
% 	}
% 	and
% 	\eq{\norm{z-\Pp_{\text{cone}(\psi_i)}(z)}^2 =\norm{z}^2\min\left(1- (\frac{\langle z,\psi_i \rangle}{\norm{z}\norm{\psi_i}})^2,1\right)
% 		}
% Therefore for a cone associated with a point cloud the projection correspond to an atom with maximal coherence.  	
% 
% 
%%(or its proximal-gradient equivalences e.g. studied in \cite{TIPHSI,BLIPsiam}) 
As a result, the IPG algorithm breaks down the computations into local updates namely, the gradient and projection steps for which an exact projection step e.g. by using a brute-force nearest neighbour (NN) search, has complexity $O(Jd)$ in time.% the closest dictionary atoms to the current solution)
%where at each iteration one requires to perform $O(Jd)$ computations to locally solve/update the problem. 


%However this linear complexity in $d$ can still be a serious bottleneck for solving problems with very large size datasets. We address this issue by replacing the exhaustive search with fast approximate searches.


%\subsection{Measurement bound}
%The classic Johnson-Lindenstrauss lemma says that one can use random linear transforms to stably embed point clouds into a lower dimension of size $O(\log(\#\widetilde \Cc))$ where $\#$ stands for the set cardinality~\cite{JL}.
%{\thm{\label{th:JL} Let $\widetilde \Cc$ be a finite set of points in $\RR^{\n}$. For $A$ drawn at random from the i.i.d. normal distribution and a positive constant $\widetilde \theta$, with very high probability one has
%		\eq{(1-\widetilde \theta)\norm{(x-x')} \leq \norm{A(x-x')}\leq (1+\widetilde \theta)\norm{(x-x')}, \quad \forall x,x' \in \widetilde \Cc
%			}
%			provided $m=O(\log(\#\widetilde \Cc)/\widetilde \theta^2)$.
%		}}
%		
%Note that this definition implies an RIP embedding for the point cloud model according to \eqref{eq:RIP} with a constant $\theta<3\widetilde \theta$ which in turn (and for small enough $\widetilde \theta$) implies the sufficient embedding conditioning for a stable CS recovery using the exact or approximate IPG (see for more details Section~\ref{sec:main}). 
%This bound considers an arbitrary point cloud and could be improved when data points $\widetilde \Cc\subseteq \Mm$ are derived from a low-dimensional structure, e.g. a smooth manifold $\Mm$ such as the MR Fingerprints, for which one can alternatively use $m=\dim_{E}(\Mm)$ for the corresponding RIP type \emph{embedding dimension} listed e.g. in \cite{RichCSreview}.
%
%%$m \propto \dim_{E}(\widetilde \Cc)\leq \n$ where $\dim_{E}(.)$ denotes the embedding dimension to satisfy RIP type embedding \eqref{eq:RIP}.
%
%% e.g. points that are living on a smooth manifold 
%%A more recent result \cite{Indyk:NNembedding} also considers the low dimensional structures within data points and weakened the measurement requirement to $m \propto \dim(\widetilde \Cc)\leq \n$ under certain conditions and notions of data intrinsic dimensionality. \todo{add embedding dims papers eg richs overview}
%
%%This $\theta$-stable embedding has similarities with the bi-Liptchitz embedding that we discussed in section x that 
%%
%%defined above, also known as the Restricted Isometry Property (RIP), is the key to guaranty the success of many CS recovery programs. For certain infinite models such as sparse (or in general the union of linear models), low-rank or smooth manifold signals the measurement bound of JL lemma can be further milden to $m \propto \dim(\Cc)$, where $\dim$ denotes the intrinsic dimensionality of the corresponding model e.g. sparsity level, rank of a matrix or manifold (intrinsic) dimension \nref [classiCS]. 
%%In relation to Definition \eqref{def:Lip}, we note that RIP is a uniform (stronger) guaranty whereas ours is local on RCS i.e.  we have $1-3\delta\leq \mmx$ and w.r.t. RLS it holds $L=1+3\delta$.
%		
%We note that such a measurement bound for a product space model  \eqref{eq:prod} and without considering any structure between spaces turns into 
%\eq{
%	m=O\left(J\min\left\{\log(d), \dim_E(\Mm)\right\}\right).
%	}
%
%\section{Discrete smooth manifold data}
%Data driven CS may also apply to algebraic models with non trivial projections. For example in the MRF reconstruction problem one first constructs a dictionary of magnetization responses (across the readout times) for many $T1,T2$ relaxation values (i.e. spin-spin and spin-echo) presented in normal tissues \cite{MRF}. This corresponds to sampling a two-dimensional manifold associated with the solutions of the \emph{Bloch dynamic  equations}~\cite{BLIPsiam}, which in the MRF settings neither the response nor the projection has an analytic closed-form solution.


==> cam_ready - arxiv2/sections/expe.tex <==

\section{Numerical Experiments}
\label{sec:expe}

\begin{figure}
	\centering
	\subfloat[Flip angles (excitations) sequence]{
		\includegraphics[width=.4\textwidth]{./figs/FISP_FA.png}
	}
	\quad
	\subfloat[Normalized MRF dictionary atoms (the real components)]{
		\includegraphics[width=.4\textwidth]{./figs/Dico_FISP.png}
	}
	\caption{TrueFISP flip angles and the corresponding normalized Bloch responses (fingerprints).\label{fig:FISP}}
\end{figure}

\begin{figure*}[!h]
	\centering
	\begin{minipage}{\textwidth}
		\centering
		\subfloat[Cover tree segments at scale 2]{\includegraphics[width=.22\textwidth]{./figs/spars/MRFtree_level2} }
		\quad
		\subfloat[Cover tree segments at scale 3]{\includegraphics[width=.22\textwidth]{./figs/spars/MRFtree_level3} }
		\quad
		\subfloat[Cover tree segments at scale 4]{\includegraphics[width=.22\textwidth]{./figs/spars/MRFtree_level4} }
		\quad
		\subfloat[Cover tree segments at scale 5]{\includegraphics[width=.22\textwidth]{./figs/spars/MRFtree_level5} }
		
		\caption{A cover tree is formed on the Bloch response manifold composed of 14 scales: (a-d) data partitions are highlighted in different colours and demonstrated for scales 2-5. Low-scale partitions  divide into finer segments by traversing down the cover tree i.e. increasing the scale.  \label{fig:CT1} }
	\end{minipage}
\end{figure*}
We investigate application of our proposed scheme for accelerating the MRF reconstruction.
Parameter estimation consists of two off-line steps: i) forming the fingerprints dictionary  by solving the Bloch dynamic  equations for a wide range of parameters. 
%This step is equivalent to sampling the 2-dimensional compact and differentiable manifold of the Bloch equation;
ii) building a cover tree structure on the resulting dictionary which enables using fast ANN searches within the iterations of the inexact IPG algorithm. 

%Since the fingerprints belong to a low-dimensional manifold (here the dimension is only 2) one would expect to achieve a better computation trade-off by using the cover tree ANN compared to the exact exhaustive search.
 

We construct a cover tree on a dictionary composed of $d=48682$  fingerprints which are
sampled from the Bloch response of $d$ pairs of $(T1, T2)$ relaxation times ranging between 100-5000 (ms) and 20-1800 (ms), respectively.\footnote{In our experiments we set the off-resonance frequency parameter to zero, the  repetition time $TR=37$ (ms) and the echo time $TE=TR/2$.}	
Fingerprints $\psi_i\in \CC^{1024}$ are normalized magnetization responses of the corresponding parameters to a balanced
steady-state free-precession (bSSFP
or TrueFISP) sequence of  1024 slowly varying flip angles (excitations) ranging from $0^\circ$
to $60^\circ$, shown in Figure~\ref{fig:FISP}. From Figure~\ref{fig:CT1} we can observe the MRF low dimensional manifold across its first three principal components. The hierarchical data partitions resulted by the cover tree is also depicted for four scales (the tree has total 14 scales with the finest coverage resolution $\sim 10^{-4}$). The ground truth image is a synthetic $256\times256$ brain phantom with six $(T1,T2)$ segments previously used for evaluations in \cite{BLIPsiam}.  Figure~\ref{fig:phantom} shows the corresponding segments, $T1$, $T2$ and proton density maps. This phantom is synthesized with the corresponding Bloch responses and proton density according to model~\eqref{eq:immodel} to build the magnetization image $X$. 
The k-space subsampling is based on a lattice-based non random EPI protocol (i.e. uniform row subselection with a  shifted pattern for different image slices). We assume no noise on the measurements and we set the step size $\mu=n/m$ in all experiments.

We apply the $(1+\epsilon)$-ANN tree search for different values of $\epsilon=\{0, 0.2, 0.4, 0.6, 0.8\}$. %At each iteration, the tree search is initialized with the current estimate per pixel (as opposed to restarting from the root). %(we refer to this algorithm as BLIP-CT). 
We compare the performances of the exact and inexact data driven IPG on this synthetic phantom. 
We only report the cost of projections i.e. the total number of pairwise distances calculated for performing the NN or ANN searches.\footnote{Since the MRF's  forward/adjoint sampling operator is based on the Fast Fourier Transform, the gradient updates cost a tiny fraction of the search step  (particularly when dealing with large-size datasets) and thus we exclude them from our evaluations.}
Results are depicted in Figure~\ref{fig:accu} and indicate that the inexact algorithm (for a suitable parameter $\epsilon$) achieves a similar level of accuracy as for the exact IPG (with an exhaustive search) by saving 2-3 orders of magnitude in computations. Using an exact tree search (i.e. $\epsilon=0$) also saves computations by an order of magnitude compared to using a brute-force search.  
Remarkably, for subsampling ratio $8:1$ the solution accuracy of the approximate scheme is about an order of magnitude better than the exact IPG. Although our theoretical results do not cover such observation, we shall relate it to a common practical knowledge that using soft decisions (e.g. here approximations)  generally improves the performance of nonconvex algorithms compared to making hard decisions, and introduces a notion of robustness against undesirable local minima in such settings.  

  



\begin{figure}
	\begin{minipage}{\linewidth}		
		\centering
		\subfloat[Brain phantom segments]{
		\includegraphics[width=.51\textwidth]{./figs/segment}
	}
	\quad\hspace{-1cm}
	\subfloat[T1 map]{
		\includegraphics[width=.51\textwidth]{./figs/T1map}
	}
		\quad
		\subfloat[T2 map]{
			\includegraphics[width=.51\textwidth]{./figs/T2map}
		}
			\quad \hspace{-1cm}
			\subfloat[Proton density map]{
				\includegraphics[width=.51\textwidth]{./figs/PDmap}
			}
		\caption{Anatomical brain phantom. Segments correspond to Background, CSF, Grey Matter, White Matter, Muscle, Skin.\label{fig:phantom}}
	\end{minipage}
\end{figure}


%============ Parameter Accuracies ====================
\begin{figure*}[t]
	\centering
	\subfloat{\includegraphics[width=.3\linewidth]{./figs/SolAccu_compres_8} }
	\quad
	\subfloat{\includegraphics[width=.3\linewidth]{./figs/T1Accu_comp_compres_8} }
	\quad
	\subfloat{\includegraphics[width=.3\linewidth]{./figs/T2Accu_comp_compres_8} }
	
		\centering
		\subfloat{\includegraphics[width=.3\linewidth]{./figs/SolAccu_compres_16} }
		\quad
		\subfloat{\includegraphics[width=.3\linewidth]{./figs/T1Accu_comp_compres_16} }
		\quad
		\subfloat{\includegraphics[width=.3\linewidth]{./figs/T2Accu_comp_compres_16} }
	
	\caption{Normalized solution MSE (i.e. $\frac{\norm{\hat x-x_0}}{\norm{x_0}}$) and  average T1, T2 errors (i.e. $\frac{1}{J}\sum_{j=1}^J |\hat T1(j) -T1(j)|$ and $\frac{1}{J}\sum_{j=1}^J |\hat T2(j) -T2(j)|$) vs. computations cost (projection step only), for two subsampling regimes. Here the  inexact IPG with $\epsilon=0.4$ achieves the lowest  solution MSE (for both subsampling regimes) among all tested methods with a clear computation cost advantage compared to the exact algorithms. %The markers 'o' and '+' correspond to the average erros in estimating T1 and T2 relaxation times, respectively.
	\label{fig:accu}}
\end{figure*}





==> cam_ready - arxiv2/sections/intro.tex <==
\section{Introduction}

Compressed sensing (CS) algorithms adopt efficient signal models to achieve accurate reconstruction given small number of non-adaptive measurements~\cite{DonohoCS, CRT:CS}. CS consists of a linear sampling model:
\eql{
	\label{eq:CSsampling}
	y \approx Ax_0,
}
where  $y$ is a noisy $m$-dimensional vector of measurements taken from the ground truth signal $x_0$ in a high dimension $n\gg m$ through using a linear mapping $A$. The success of CS for stably inverting such ill-posed systems relies on the fact that natural signals often follow low-dimensional models $\Cc$ with limited degrees of freedom compared to their original ambient dimension, and that certain random sampling schemes can compactly (in terms of the measurements) preserve the key signal information (see e.g.~\cite{RichCSreview} for an overview on different CS models and their corresponding sample complexities). 
Variational approach for CS reconstruction consists of solving e.g. the following constrained least-square problem:
\eql{\label{eq:opt1}
	\hat x = \argmin_{x \in \Cc} \norm{y-Ax}_2^2.
}  
where the constraint takes into account the signal model.


%CS finds a wide applications in e.g. biomedical imaging, astrophysics, remote sensing just to name few~\nref. 
% The success of CS heavily relies on the fact that natural signals often have limited degrees of freedom as compared to their original ambient dimensionality and on the other hand certain random sampling schemes e.g. i.i.d. subgaussian distributions, random orthoprojectors, fast Johnson-Lindenstrauss transoms,..., can compactly (in terms of the measurements) preserve the key signal information required for a stable inversion/recovery. 
% In this regard the number of CS measurements scale sub-linearly with the signal ambient dimension and is proportional to the intrinsic dimension (see \cite{DonohoCS, CRT:CS,Tropp:SOMP1,Candes:EMC,BW:manifold,modelbasedCS} and e.g. \cite{RichCSreview} for an overview on different CS models and their corresponding measurement complexities). And thus incorporating the low-dimensional signal structure is proven to significantly help with an accurate inference in the noisy and undersampled regimes. 

%The CS reconstruction algorithms are in general more computationally complex (as opposed to the simple linear acquisition of CS) as they require to handle  mostly non-linear and complicated models. 
First order methods based on iterative local gradient and projection (or also proximal) updates 
%\eql{\label{eq:IPGD}
%	x^{k+1} = \Pp_{\Cc} \left( x^{k} - \mu A^H(Ax^{k}-y) \right) 
%}
are popular for CS recovery due to their scalability for big data  problems~\cite{Volkan:bigdata} and their flexibility in handling various complicated (convex/nonconvex and sometimes combinatorial) models~\cite{Blumen}. Starting from an initial point e.g. $x^{k=0}=\mathbf{0}$  and for a given step size $\mu$, the solution of Iterative Projected Gradient (IPG)  iteratively updates as follows:
\eql{\label{eq:IPGD}
	x^{k+1} = \Pp_{\Cc} \left( x^{k} - \mu A^H(Ax^{k}-y) \right), 
}
where the projection is defined as $\Pp_\Cc(x)\in \argmin_{u\in\Cc}\norm{x-u}$ and throughout, $\norm{.}$ stands for the Euclidean norm.

%The following embedding assumption 
%%(with a ratio $\approx 1$ between the constants) 
%guarantees a stable CS inversion for an arbitrary signal model $\Cc$ (possibly nonconvex) using the IPG algorithm: 
%{\defn{\label{def:bilip} $A$ is Bi-Lipschitz w.r.t. $\Cc$, if $\forall x,x'\in \Cc$ there exists constants $0<\alpha\leq \beta$ such that
%		\eql{\label{eq:bilip}
%			\alpha \norm{x-x'}^2 \leq \norm{A(x-x')}^2\leq \beta \norm{x-x'}^2  }	
%	}}
%It has been shown in that if $\beta/\alpha<2$ then IPG  $(A,\Cc)$ is a bi-Lipschitz embedding with w.r.t. $C$The stability of the IPG 
%
%Dealing with complicated signal models, the projection step can bring a huge computational burden at each iteration.
%
%Recently it has been shown that IPG is also robust to $(1+\epsilon)$-approximate projections.



In this work we consider compressed sensing of signals living on a low-dimensional smooth manifold. In this case, the model projection might not be computationally easy for certain complex manifolds. A popular approach consists of collecting discrete samples of the manifold in a dictionary~\cite{recht:discretize,SCOOP}, i.e. a \emph{data driven} CS approach,  and approximate the projection step by searching the nearest atom in this dictionary.  Depending on the manifold complexity and the desired approximation accuracy, the size of this dictionary can be very large in practice. In this case performing an \emph{exhaustive} nearest neighbour (NN) search could become computationally challenging. % the nearest matching step. 

We address this shortcoming by preprocessing the dictionary and build a tree structure suitable for fast \emph{approximate} nearest neighbour (ANN) searches. Recently, it as been shown 
%that under the embedding assumption IPG is robust against approximations and
that provided enough measurements and for moderate approximations the \emph{inexact} IPG achieves similar solution accuracy as for the exact algorithm~\cite{me:inexactIPG}. 
In this regard, we use the \emph{cover tree} structure~\cite{beygelzimer2006cover,Navigating} which is proposed for fast ANN searches on large datasets with low intrinsic dimensionality and with a search complexity $O(\log(d))$ in time, where $d$ is the dataset population (in contrast with the linear complexity of an exact exhaustive search $O(d)$). %The theory predicts that provided enough measurements and for a suitably chosen approximation parameter  the solution accuracy is the same as for the exact algorithm. 

We apply our results to accelerate the Magnetic Resonance Fingerprint (MRF) recovery from under-sampled k-space measurements; an emerging field of study in computational medical imaging~\cite{MRF}. 
%Recently an iterative exact projection algorithm (BLIP) is proposed for the MRF problem~\cite{MRF} that achieves the state-of-the-art trade-off in parameter estimation accuracy vs. compression~\cite{BLIPsiam}. At each iteration, BLIP performs an exhaustive search to find the closest fingerprint to the current estimate, and thus its running time linearly increases for larger fingerprint dictionaries i.e. of size $\sim O(10^6)$ atoms in certain practical setups. 
%
Since the MR fingerprints belong to the low-dimensional manifold of Bloch dynamic equations, we show that using the cover tree ANN search significantly shortcuts the computations compared to an exact IPG with exhaustive searches as in~\cite{BLIPsiam}.  
%Indeed, we address this shortcoming by using cover tree's fast approximate search. 
%We implement this algorithm 
%and compare it with the exact IPG algorithm previously proposed for this problem~\cite{BLIPsiam},  
%(iterative Projection Accelerated with Cover Tree Search). 
%Note that our preprocessing includes an additional step of forming a cover tree on the fingerprints.
%and for a similar reconstruction accuracy, we report 2-3 orders of magnitude reduction in the total projection cost compared to an exact IPG algorithm previously proposed for this problem~\cite{BLIPsiam} based on exact brute-force NN searches. 




% It has been proven that    
%
%$X = \{x_i\}_i$ belong to a manifold $\Mm$ with low intrinsic dimensionality. Given small number of measurement that are  linear combination of the signals $\{y_j\}_{j=1:m}$, where $y_j =\sum_i A_{j,i} x_i$  we would like to find $X$. 

\section{Preliminaries}
The following embedding assumption plays a critical role in stability analysis of the (convex/nonconvex) IPG algorithm~\cite{BW:manifold,Blumen,me:inexactIPG}:
%(with a ratio $\approx 1$ between the constants) 
%guarantees a stable CS inversion for an arbitrary signal model $\Cc$ (possibly nonconvex) using the IPG algorithm: 
{\defn{\label{def:bilip} $A$ is bi-Lipschitz w.r.t. $\Cc$, if $\forall x,x'\in \Cc$ there exists constants $0<\alpha\leq \beta$ such that
		\eql{\label{eq:bilip}
			\alpha \norm{x-x'}^2 \leq \norm{A(x-x')}^2\leq \beta \norm{x-x'}^2  }	
	}}
Dealing with complicated signal models, the projection step can bring a huge computational burden at each iteration, and thus a natural line of thought is to perform this step with cheaper (available) approximations. The inexact IPG takes the following form:
\eql{\label{eq:inIP2}
	x^k = \Pp_\Cc^{\epsilon}\left(x^{k-1}-\mu A^H(Ax^{k}-y) \right).}
We consider the class of $(1+\epsilon)$-approximate projections: for any $\epsilon\geq0$:
\eql{\label{eq:eproj}
	\Pp_\Cc^{\epsilon}(x) \in \Big\{ u\in \Cc :\,	\norm{u-x} \leq (1+\epsilon)\norm{\Pp_\Cc(x)-x}  \Big\}. 
}
The following result states that if the embedding holds (with a better conditioning compared to the exact IPG case $\epsilon=0$) then the inexact algorithm  still achieves a solution accuracy comparable to the exact IPG~\cite{me:inexactIPG}:
{\thm{\label{th:inexactLS2} Assume $(A,\Cc)$ is bi-Lipschitz, $\xgt\in \Cc$ and that
		\eq{\sqrt{\epsilon+\epsilon^2}\leq \delta\sqrt{\mmx}/{\vertiii{A}} \qandq \MM < (2-2\delta+\delta^2) \mmx} 	
		for $\epsilon\geq 0$ and some constant $\delta \in [0,1)$.
		Set the step size $\left((2-2\delta+\delta^2) \mmx\right)^{-1}<\mu\leq\MM^{-1}$. The sequence generated by Algorithm \eqref{eq:inIP2} obeys the following bound:
		\eq{
			\norm{x^{k}-\xgt}\leq  \rho^k \norm{\xgt} + 
			%\frac{ \left( 2\frac{\sqrt{M}}{m}+\frac{\sqrt\mu}{\norm{A}}\delta \right)}
			\frac{\kappa_w}{1-\rho}w
		}
		where 
		\begin{align*}
		\rho=\sqrt{\frac{1}{\mu \mmx} -1}+ \delta, \quad
		\kappa_w= 2\frac{\sqrt{\MM}}{\mmx}+\sqrt\mu\delta, \quad
		w=\norm{y-A \xgt}.
		\end{align*}		
		
	}} 	
	{\rem{Increasing $\epsilon$ slows down the rate $\rho$ of linear convergence, however the iterations are potentially cheaper. Too large approximations $\epsilon$ may result in divergence.}}
	{\rem{After a finite $K=O(\log(\tau^{-1}))$ number of iterations Algorithm \eqref{eq:inIP2} achieves the solution accuracy $\norm{x^K-x_0}=O(w)+\tau$, for any  $\tau>0$.}}





==> cam_ready - arxiv2/sections/manifCS.tex <==
\section{Manifold Compressed sensing}
\label{sec:ManifCS}
\subsection{Exact iterative projected gradient}
Compressed sensing consists of a linear sampling model
\eql{
	\label{eq:CSsampling}
	y \approx Ax_0,
}
where  $y$ is a noisy $m$-dimensional vector of measurements taken from signal $x_0$ in a high dimension $n\gg m$ through using a linear mapping $A$.%and the vector $w$ accounts for bounded noise corruptions.
Variational approach for CS recovery consist in solving following program:
\eql{\label{eq:opt1}
	x^{opt} = \argmin_{x \in \Mm} \norm{y-Ax}_2^2.
}  
First order methods in form of Iterative Projected Gradient (IPG) are very popular to solve \eqref{eq:opt1}. Each iteration has a gradient update followed by a Euclidean projection onto the model $\Mm$ defined as 
\eq{\Pp(x) := \argmin_{u\in\Mm} \norm{u-x}_2^2.}
Starting from the initial point $x^{k=0}=0$, the solution of IPG iteratively updates as follows
\eql{\label{eq:IPGD}
	x^{k+1} = \Pp_{\Mm} \left( x^{k} - \mu A^H(Ax^{k}-y) \right) 
}
until it convergences. % \rightarrow \hat{x} $.	
A general convergence result holds for both convex and non-convex constraints $\Mm$, that is by choosing the step size small enough $\gamma\leq 1/\norm{A}$, IPG converges to a critical point of the problem \eqref{eq:opt1} which for convex $\Mm$ is also a global convergence i.e., $\lim{x^{k}}\rightarrow x^{opt}$.  \nref ATOUCH. 


Remarkably a different line of result guarantees that IPG can globally solve \eqref{eq:opt1} even for the non-convex $\Mm$ constraints. The key assumptions here are the following embedding property and a related properly chosen lower bound on the step size $\mu$.
{\defn{\label{def:bilip} $A$ is Bi-Lipschitz w.r.t. $\Mm$, if $\forall x,x'\in \Mm$ there exists constants $0<\alpha\leq \beta$ such that
		\eql{\label{eq:bilip}
			\alpha \norm{x-x'}^2 \leq \norm{A(x-x')}^2\leq \beta \norm{x-x'}^2  }	
}}
{\thm{\label{th:exactIPG}
[Blumensath'11] Assume $A$ is bi-Lipschitz w.r.t. $\Mm$ and $\xgt\in \Mm$ with constants satisfying $\MM < 1.5\mmx$. Set the step size $2/3\mmx^{-1}<\mu\leq\MM^{-1}$. The sequence generated by IPG Algorithm \eqref{eq:IPGD} obeys the following bound:
		\eql{\label{eq:errbound}
			\norm{x^{k}-\xgt}\leq  \rho^k \norm{\xgt} + \frac{2\sqrt{\MM}}{\mmx(1-\rho)}w
		}
		where,  	
		$\rho=\sqrt{\frac{1}{\mu \mmx} -1}$ 
and $w=\norm{y-A\xgt}$.
}}
\subsection{Iterative approximate projected gradient}
For computational reasons one sometimes requires to consider an approximate model projection. This particularly applies to very complex models where the exact projection is not explicit and amounts to solving an auxiliary optimization at each iteration (or for instance conducting an expensive exhaustive search as will be later discussed in the MRF application). Fortunately the IPG algorithm is shown to be robust against approximations. We define below a widely applicable notion of near-optimal approximation for the projection step:

{\defn{ The $(1+\epsilon)$-approximate projection is defined as follows and for a given $\epsilon\geq0$:
\eql{\label{eq:eproj}
	\pp_\Mm^{\epsilon}(x) \in \Big\{ u\in \Cc :\,	\norm{u-x} \leq (1+\epsilon)\norm{\pp_\Cc(x)-x}  \Big\}. 
}
We note that $\pp_\Mm^{\epsilon}(x)$ might not be unique.}}

 In this regard, the inexact IPG algorithm with a $(1+\epsilon)$-approximate projection takes the following form:
\eql{\label{eq:inIP2}
	x^k = \pp_\Mm^{\epsilon}\left(x^{k-1}-\mu A^H(Ax^{k}-y) \right).}
The following result states that if the embedding holds (with a better conditioning compared to the exact IPG case) then the inexact algorithm  still achievs the accuracy of the exact IPG.

{\thm{\label{th:inexactLS2} Assume $A$ is bi-Lipschitz w.r.t. $\Mm$ and $\xgt\in \Mm$ and that
\eq{\sqrt{\epsilon+\epsilon^2}\leq \delta\frac{\sqrt{\mmx}}{\vertiii{A}} \qandq \MM < (2-2\delta+\delta^2) \mmx} 	
for $\epsilon\geq 0$ and some constant $\delta \in [0,1)$.
		Set the step size $\left((2-2\delta+\delta^2) \mmx\right)^{-1}<\mu\leq\MM^{-1}$. The sequence generated by Algorithm \eqref{eq:inIP2} obeys the following bound:
		\eq{
			\norm{x^{k}-\xgt}\leq  \rho^k \norm{\xgt} + 
			%\frac{ \left( 2\frac{\sqrt{M}}{m}+\frac{\sqrt\mu}{\norm{A}}\delta \right)}
			\frac{\kappa_w}{1-\rho}w
		}
		where 
		\begin{align*}
		\rho=\sqrt{\frac{1}{\mu \mmx} -1}+ \delta, \quad
		\kappa_w= 2\frac{\sqrt{\MM}}{\mmx}+\sqrt\mu\delta, \quad
		 w=\norm{y-A \xgt}.
		\end{align*}		
		
	}} 	
	{\rem{Increasing $\epsilon$ limits the recovery guaranty and slows down the convergence (by comparing $\rho$ in Theorems 1 and 2).}}


\subsection{Manifold embedding results}
The embedding holds when $A$ drawn at random from certain distributions (e.g. element-wise i.i.d. subgaussian, or random row selection of orthonormal bases) and when number of the measurements $m \approx O(\dim(\Mm))$. 

{\thm{[Wakin, Baraniuk'09] Let $\Mm\in \RR^n$ be a compact Riemannian manifold with dimension $\dim(\Mm)$, condition number $1/\tau$, volume $V$ and Geodesic regularity $R$. Then a random orthoprojector $A\in\RR^{m\times n}$ with probability $1-\xi$ provides a bi-Lipschitz embedding on $\Mm$ with $\mmx=1-\theta, \MM=1+\theta$, given 
\eql{
	m=O\Big(\dim(\Mm)\log(nVR\tau^{-1})\theta^{-2}\log(\xi^{-1})\Big)
	}		
for positive constants $\xi,\theta<1$.
}}
		
Embeddable manifolds:
\begin{itemize}
	\item Smooth manifolds with bounded condition number $1/\tau$ \nref[Richwakin][Clarkson]
	\item Doubling sets with finite resolution $\forall x,x'\in \Mm \norm{x-x'}>\Delta_{\min}$ \nref[Indyk'08].
	\item Smooth manifolds are doubling\nref[Dasgupta'12].   
\end{itemize}
%\todo{Results for manifold IPGD, with that perhaps others can be more summerized} 
\subsection{Discretization}\label{sec:discrete}
In this part we consider compressed sensing of signals living on a compact \emph{discrete} manifold $\Mb$ with low intrinsic dimension. The set $\Mb$ may be a dense collection of samples from a continuous manifold with a non trivial projection.
% As the projection step might not be trivial or computationally easy for many complex manifolds we consider a data driven approach which consists of collecting discrete samples of the manifold in a dictionary and approximate 
With such formalism the projection step reduces to searching the nearest atom, however (potentially) in a very large dictionary. 
%With such formalism, the size of discrete manifold $\Mb$ may very large, bringing both storage and computational concerns to the nearest matching step.
This is also related to the \emph{Data driven} compressed sensing framework (with applications in e.g. Hypercritical imagery \cite{TIPHSI}, Mass spectroscopy \nref, MALDI imaging \cite{Kobarg2014}) where in absence of an algebraic physical model one resorts in collecting a large number of data samples in a dictionary and use it as a \emph{point cloud} model for CS reconstruction~\cite{RichCSreview}.  

%In this case the model is $\Mm = \bigcup_{i=1}^{d}\{\psi_i\}$ where $\psi_i\in\RR^n$s are atoms of a $n\times d$ dictionary $\Psi$. %\{\psi_i\}_{i=1}^{d}$
% of $d$ points (atoms) in $\RR^n$ the model becomes.  
%Data driven CS finds numerous applications e.g. in Hypercritical imagery \cite{TIPHSI}, Mass spectroscopy \nref, MALDI imaging \cite{Kobarg2014} and Magnetic Resonance Fingerprinting (MRF)~\cite{MRF,BLIPsiam} just to name a few\todo{add more}. For instance the USGS Hyperspectral library \footnote{\url{http://speclab.cr.usgs.gov}} contains the spectral signatures (reflectances) of hundreds of substances measured across $\sim 400$ frequency bands. This side information is shown to be useful for CS reconstruction and classification in both convex and nonconvex settings (see e.g. \cite{TIPHSI} for more details and its relations to sparse approximation in redundant dictionaries).  
%Recently MR Fingerprinting~\cite{MRF} proposed a fast CS acquisition scheme for quantifying the NMR properties (such as the $T1,T2$ relaxation times, off-resonance frequencies, proton density) of tissues. Since random excitation sequences generate magnetization responses in non-analytic forms, \cite{MRF} proposed build a very large dictionary of fingerprints driven by the Bloch dynamic equations for all combination of those parameters. 

Data driven CS may also apply to algebraic models with non trivial projections. For example in the MR Fingerprinting problem one first constructs a dictionary of magnetization responses (across the readout times) for many $T1,T2$ relaxation values presented in normal tissues \cite{MRF}. This corresponds to sampling a two-dimensional manifold associated with the solutions of the \emph{Bloch dynamic  equations}, which in the MRF settings neither the response nor the projection has a analytic closed-form solution. In this setting the discrete model reads
\eql{\label{eq:discrete}
	\Mb:=\bigcup_{i=1}^{d}\{\psi_i\} \in \RR^J}
that is a point cloud model associated with atoms of a dictionary $\Psi$ customized for e.g. HSI, MALDI or MRF data.

In a single dimensional setting 
i.e. when $x$ is a vector in $\RR^n$  there will be no need for an IPG algorithm to solve problem \eqref{eq:opt1} for a discrete model $\Mm=\Mb$. In fact if the embedding i.e. Definition~\ref{def:bilip} holds with a $\mmx>0$, then a \emph{single step} nearest neighbour matching can solve the problem with a noise robustness depending on the constant $\mmx$.


%the set $\Mm$ may also be a dense collection of samples from a continuous algebraic manifold with a non trivial projection e.g. Magnetic resonance fingerprinting \nref. 
% As the projection step might not be trivial or computationally easy for many complex manifolds we consider a data driven approach which consists of collecting discrete samples of the manifold in a dictionary and approximate 




%Recently MR Fingerprinting \cite{MRF} proposed a fast CS acquisition scheme for quantifying the NMR properties (namely the $T1,T2$ relaxation times) of tissues. Small number of  excitations in form of rotating the magnetic field applies to the tissue, and between each two excitations, the \emph{partial} k-space information is measured. An iterative exact projection algorithm (BLIP) is proposed for the MRF problem which achieves a great parameter estimation accuracy \cite{BLIPsiam}. % versus compression trade-off $\nref$.
%The projection consists of NN searches on a densely sampled manifold $\Mb$ of fingerprints driven by the Bloch dynamic equations.



==> cam_ready - arxiv2/sections/mrf_part.tex <==
\section{Application in Quantitative MRI}


%The main body of measurements in MR imaging comes from the net magnetic moment of proton spins in a given voxel.
%Excitations in form of rotating the external magnetic field, referred to as Flip Angles (FAs), apply at certain time intervals. Proton spins respond to these excitations; they get aligned with the new field and yet, relax back to the equilibrium state however non-instantaneously. 
%Two exponents characterize the time proton magnetization takes to reach equilibrium: i) the \emph{spin-lattice} longitudinal relaxation $T1$, 
%%the exponent related to the time for longitudinal magnetization component to recover, 
%and ii) the \emph{spin-spin} transverse relaxation $T2$. These exponents are unique for biological tissues.

In \emph{quantitative MRI} 
%(in contrast with single image qualitative MRI) 
rather than simply forming a single MR image with only  contrast information (i.e. qualitative MRI), physicists
are interested in measuring the NMR properties of tissues   namely, the $T1,T2$ relaxation times, $\delta f$ magnetic resonance and proton density (PD), and use these parameters to differentiate different biological tissues~\cite{toftsqmri}. The standard approach for parameter estimation is to acquire a large sequence
of images in different times from a simple excitation pulse (i.e. excitations in terms of rotating the magnetic field)  and then use an exponential model curve fitting to recover the decay exponents $T1,T2$ for each voxel. This procedure runs separately to estimate each relaxation time.
The long process of acquiring multiple fully sampled images, brings serious limitation to standard approaches in quantitative imaging to apply within a reasonable time and with an acceptable signal-to-noise ratio (SNR) and resolution.
%
%These procedures are 
% \eqref{eq:mrf-decay1} and \eqref{eq:mrf-decay2} see for instance \nref [Wajiha's]. 
% 
%%which characterizes decay of the transversal component.
%More formally, for $\m(t)=[\m^x(t) \, \m^y(t) \, \m^z(t)]^T$ the magnetization vector at time $t$ we have:
%\begin{align}
%\m^z (t)&= \m^z_{eq} - \left(\m^z_{eq}-\m^z(0)\right)e^{-t/{T1}}, \label{eq:mrf-decay1}\\  
%\m^{xy}(t) &= \m^{xy}(0)e^{-t/{T2}}.\label{eq:mrf-decay2}
%\end{align}
%Interestingly, different molecular structures have distinct $T1,T2$ relaxations. For instance, it has been discovered in '70s that tumours have higher $T1$ relaxation times than normal tissues.
%%; a discovery which brings huge attention to such characterization since 1971. 
%Since then more studies have established relating certain neurological degradations (causing brain disorders e.g. MS) to anomalies observed in relaxation times, which ultimately established a whole field of study known as \emph{quantitative MRI}:
%Rather than simply forming a single MR image that measures
%the transverse magnetization response, physicists
%measure the NMR properties of tissue namely, $T1,T2$ and proton density (PD), and use these parameters to differentiate different biological tissues\nref [paul Toft book]. The standard approach for parameter estimation is to acquire a large sequence
%of images in different times from an initial excitation pulse, and then use exponential curve fitting to recover $T1,T2$ per voxel using models \eqref{eq:mrf-decay1} and \eqref{eq:mrf-decay2} see for instance \nref [Wajiha's]. 


\subsection{Magnetic Resonance Fingerprinting}



Recently, a novel parameter estimation process coined as the \emph{Magnetic Resonance Fingerprinting} (MRF) has been proposed to address this shortcoming. 
For the acquisition, MRF applies a shorter sequence of random excitations (i.e. $\Gamma \in [0,\pi/2]^{\n}$ random flip angels with  typically $\n\approx 300-1000$ and the time interval $TR\sim 10-40$ msec) for estimating all parameters $T1,T2,\delta f$, and proton density at once.
%\item This sequence can be further optimized and shortened w.r.t. the random choice of FAs, see \nref [Cohen'15, Mahbub'16].
 After each excitation pulse the response is recorded  through the 
measurements taken from a small portion of k-space.
%\end{itemize} 
As a result the acquisition time can significantly decreases to a couple of minutes \cite{MRF}.   

The exponential model as for the traditional acquisition sequences will no longer hold for the MRF model. Due to using random excitations, the signatures casts a non-trivial implicit expression  readable by solving the \emph{Bloch dynamic equations} $\Bb(\Gamma,\Theta)\in \CC^\n $ customized for the set of parameters $\Theta=\{T1,T2,\delta f\}$. 
The MRF problem is an example of data driven CS model with an algebraic signal model (i.e. the Bloch equations) but a non-trivial projection. For this problem one constructs off-line a
dictionary of \emph{fingerprints} (i.e. magnetization responses) for all possible $d=\#\{\Theta_i\}_i$ parameters presented in normal tissues where the atoms $\psi_i:=\Bb(\Gamma,\Theta_i)$ uniquely represent the underlying set of parameters $\Theta_i$ . This corresponds
to sampling a low-dimensional manifold associated with the
solutions of the Bloch dynamic equations~\cite{BLIPsiam}, which for complicated excitation patterns neither the response nor the projection has an
analytic solution.


%These signatures are calculated off-line for all possible $d=\#(\Theta)$ parameters and saved in a huge dictionary of \emph{fingerprints} whose atoms $\psi_i:=\Bb(\Gamma,\Theta_i)$ uniquely represent the underlying set of parameters $\Theta_i$. 


\subsection{MRF image model and parameter estimation}

%The underlying MRF image is a 3-dimensional tensor. By matricization 
An MRF image can be represented by a matrix $X\in \CC^{ \n\times J}$. Each column $X_j$ represents a $\n$-dimensional spatial pixel $j$ and each row $X^l$  represents a temporal image slice (with the spatial resolution equal to $J$) corresponding to the measurements taken after the excitation pulse $\Gamma_l$, $\forall l=1,\ldots,\n$. The total spatio-temporal resolution of the MRF image is $n:=\n J$. By the pixel purity assumption, the image follows the product space data driven model \eqref{eq:dmodel} and \eqref{eq:immodel} where each column/pixel $j$ correspond to a single fingerprint $\psi$ with a unique parameter  $\Theta$. The cone($\widetilde \Cc$) corresponds to the fingerprints dictionary and $\rho>0$ represents the proton density.\footnote{The proton density can be generally a complex number for which only the rescaling step of the cone projection slightly changes and the rest of the analysis similarly holds, for more details see~\cite{BLIPsiam}. %but here for simplicity we assume it to be a positive real number, although a similar analysis applies for the complex case~\cite{BLIPsiam}.
	} 
The MRF acquisition model is linear as follows:
\eql{\label{eq:CSMRF}	
	Y^l \approx \Ff_{\Omega_l} (X^l), \quad \forall l=1,\ldots \n,
}
where  $\Ff$ denotes the two-dimensional Fourier transform, and $\Ff_{\Omega_l}: \CC^J \rightarrow \CC^{m/\n}$ subsamples the k-space coefficients of the  image slice $X^l$ according a pattern/set $\Omega_l$.  The k-space subsampling could correspond to a spiral pattern~\cite{MRF} or a random horizontal/vertical line subselection~\cite{BLIPsiam} e.g. in the Echo Planar Imaging (EPI). %, from the 2-dimensional spatial Fourier domain.  
By vectorization of $X,Y$, we have a product space CS model similar to~\eqref{eq:CSsampling} for a sampling protocol $A$ acting spatially however with different k-space sampling pattern per image slice. 
%is $A=\Ff_{\Omega_i}\otimes I_J$ for $\otimes$ denoting the Kronecker product.

%Projection onto the Bloch manifold $\Bb$ is non-trivial for a random FA pattern (as neither the manifold nor and the projection are explicitly given). The MRF framework addresses this bottleneck with model discretezation of as explained in Section~\ref{sec:discrete}. One has to solve the Bloch equations for $d$ number of discretized parameters $\Theta$, and yet store the outcome Bloch response signature $\psi_j$ in a dictionary $\Psi$ corresponding to~\eqref{eq:discrete}. This is a preprocessing step and potentially can lead to a very large size dictionary with $d\sim O(10^6)$ atoms! Therefore in a sense the MRF framework sacrifices the memory in order to enable/facilitate the projection step of IPG.

The CS reconstruction proposed by~\cite{BLIPsiam} is based on a data driven IPG algorithm (with the \emph{exact} cone projection described in Section~\ref{sec:datadrivenCS}) where one by identifying the correct fingerprint per pixel $X_j$ can recover the underlying parameters $\Theta$ stored in a look-up table (the last rescaling step also recovers the proton density $\gamma_j$). 
It has been shown in~\cite[Theorem 1]{BLIPsiam} that if $\Omega_l$ independently at random subselects the rows (or columns) of the k-space, which corresponds to a \emph{random EPI sampling protocol}, the resulting forward map $A$ is bi-Lipschitz  w.r.t. the product model $\Cc=\prod_{j=1}^J \text{cone}(\widetilde \Cc)$, provided sufficient \emph{discriminations} between the fingerprints.\footnote{One achieves a suitable discrimination between the MR fingerprints by e.g. choosing the random excitation sequence long enough.} This result guarantees stability of the parameter estimation using this algorithm with an step size $\mu=n/m$.

Since the Bloch manifold is parametrized by only three parameters in $\Theta$ and thus has a low intrinsic dimension, we use the cover tree ANN searches to accelerate the projection step. We perform the following procedure iteratively until convergence:
\begin{align*}\label{eq:BLIP}
(X^l)^{k+1} = 
\Pp^{\epsilon}_{\text{cone}(\widetilde \Cc)} \left( (X^l)^{k} - \mu \Ff^H_{\Omega_l}\left(\Ff_{\Omega_i} ((X^l)^{k})  -Y^l\right) \right) 
\end{align*}
The approximate cone projection follows the update in~\eqref{eq:ANN1}. 


Provided with the same embedding result (for the random EPI acquisition protocol) and according to Theorem~\ref{th:inexactLS2} we can deduce the linear convergence of this algorithm to the true solution for mildly-chosen approximations $\epsilon$ (and the same step size $\mu=n/m$) where the projection step has now the complexity $O(J\log(d))$. For large-sized dictionaries the gap between the computation costs of the exact and  inexact IPG algorithm can be significantly large. %and a well-chosen step size e.g. $\mu \approx m/n$. And as consequence one achieves an exact parameter $\Theta$ estimation.




==> sections/CSIPA.tex <==
\section{Iterative approximate projected Gradient}
\label{sec:CSIPA}


\subsection{Approximate projection} 
For saving computations, we consider each iteration of \eqref{eq:IPGD} calculates an approximate (inexact) projection step.
% For that we require to first define the set of $\varepsilon$-close projections of x onto $\Mm$ as follows:   
%\eq{
%\Pp_\Mm^{\epsilon}(x) := \{ z\in \Mm :\,	\norm{z-x}^2 \leq \inf_{z'\in \Mm} \norm{z'-x}^2 + \epsilon \}
%}.
%
%For a nonempty $\Mm$ Blumensath \nref showed that $\Pp_\Mm^{\epsilon}(.)$ is nonempty.
%Then, by $\pp_\Mm^{\epsilon}(x)$ we denote a point $p\in \Mm$ belonging to that set:
%\eq{
%\pp_\Mm^{\epsilon}(x) := p \in \Pp_\Mm^{\epsilon}(x).
%}
%
For that we first define the notion of $\epsilon$-close projection of x onto $\Mm$ 
\eql{\label{eq:eproj}
	\Pp_\Mm^{\epsilon}(x) \in \{ u\in \Mm :\,	\norm{u-x}^2 \leq \inf_{u'\in \Mm} \norm{u'-x}^2 + \epsilon \}.
}
Note that the point $\Pp_\Mm^{\epsilon}(x)$ may not be unique but for a nonempty $\Mm$ it exists (see \nref Blumensath also care must be taken when $\epsilon\rightarrow 0$). 

We update the algorithm \eqref{eq:IPGD} to the following \emph{inexact IPGD} version:
\eql{\label{eq:eIPGD}
	x^{t+1} = \Pp_\Mm^{\epsilon_{t}} \left( x^{t} - \mu A^*(Ax^{t}-y) \right). 
}
where $\epsilon_t$ denotes the level of approximation for calculating  the projection step at iteration $t$.


\subsection{Convergence result}
Assume $A$ satisfies Bi-Lipschitz property with respect to $\Mm$ with constants $\alpha,\beta$ defined as follows. 


\marginpar{we don't need universal $\alpha$..just $\alpha_{x_0}$. Not same argument for $\beta$ tho}
{\thm Assume $A$ is Bi-Lipschitz w.r.t. $\Mm$ with constants satisfying $\beta < 1.5\alpha$. For the step size $\mu$ chosen so that $2/3\alpha^{-1}<\mu\leq\beta^{-1}$, the sequence generated by Algorithm \eqref{eq:eIPGD} obeys the following bound:
	%generates a sequence the solution of $\epsilon$-IPGD after $t$ iterations satisfies:
	\begin{align}
&\norm{x^{t}-x_0}^2 \nonumber \\
&\leq \rho^t  \left( \norm{x^{init}-x_0}^2 +   \frac{2}{\mu\alpha}\sum_{i=0}^{i=t} \rho^{-i} \epsilon_i \right) + \frac{4(1-\rho^t)}{\alpha(1-\rho)}\norm{w}^2. 
\end{align}
Where $\rho= 2\left(\frac{1}{\mu\alpha}-1 \right)$, and $e$ denotes the noise in the forward model  i.e. $w=y-Ax_0$.
	}

\begin{proof}
Set $g = 2A^*(Ax^t-y)$ i.e. the gradient of $\norm{y-Ax^{t}}^2$. Then we have	
\begin{align*} 
	&\norm{y-Ax^{t+1}}^2-\norm{y-Ax^{t}}^2	\\
	&= \langle x^{t+1}-x^t,g \rangle +\norm{A(x^{t+1}-x^t)}^2 \\
	&\leq \langle x^{t+1}-x^t,g \rangle + \beta \norm{x^{t+1}-x^t}^2, 
\end{align*}
where the last inequality follows from the Bi-Lipschitz property \eqref{eq:bilip} of $A$. Assuming $\beta \leq 1/\mu$, we have
\begin{align*}
&\langle x^{t+1}-x^t,g \rangle + \beta \norm{x^{t+1}-x^t}^2 \\
 & \leq \langle x^{t+1}-x^t,g \rangle + \frac{1}{\mu} \norm{x^{t+1}-x^t}^2\\
& = \frac{1}{\mu} \norm{x^{t+1}-x^t+\frac{\mu}{2} g }^2 - \frac{\mu}{4} \norm{g}^2 .
\end{align*}
Because of \eqref{eq:eIPGD}, \eqref{eq:eproj} and the fact that $x_0\in\Mm$ we have
\eq{
	\norm{x^{t+1}-x^t+\frac{\mu}{2} g }^2 \leq  \norm{x_0-x^t+\frac{\mu}{2} g }^2 +\epsilon_t.	
}
Therefore we can write
\begin{align}
&\norm{y-Ax^{t+1}}^2-\norm{y-Ax^{t}}^2 \nonumber	\\
%&=\langle x^{t+1}-x^t,g \rangle + \frac{1}{\mu} \norm{x^{t+1}-x^t}^2 \nonumber\\
&\leq \frac{1}{\mu} \norm{x_0-x^t+\frac{\mu}{2} g }^2 - \frac{\mu}{4} \norm{g}^2 +\frac{\epsilon_t}{\mu} \nonumber \\
&= \langle x_0-x^t,g \rangle + \frac{1}{\mu} \norm{x_0-x^t}^2 +\frac{\epsilon_t}{\mu} \label{eq:p1b2}
\end{align}



Similarly we can use the lower Bi-Lipschitz constant to obtain an upper bound on $ \langle x_0-x^t,g \rangle$:
\begin{align*} 
\norm{ \underbrace{y-Ax_0}_{w}}^2-\norm{y-Ax^{t}}^2	&= \langle x_0-x^t,g \rangle +\norm{A(x_0-x^t)}^2 \\
&\geq \langle x_0-x^t,g \rangle + \alpha \norm{x_0-x^t}^2.
\end{align*}
Using this bound in \eqref{eq:p1b2} and cancelling $-\norm{y-Ax^t}^2$ from both sides of the inequality, we can deduce
\begin{align*}
&\norm{y-Ax^{t+1}}^2 \leq \left(\frac{1}{\mu}-\alpha \right)\norm{x^t-x_0}^2 + \norm{w}^2+ \frac{\epsilon_t}{\mu}.
\end{align*}
Finally we use again the lower Bi-Lipschitz constant to lower bound  $\norm{y-Ax^{t+1}}^2$:
\begin{align*}
&\alpha\norm{x^{t+1}-x_0}^2\leq \norm{A(x^{t+1}-x_0)}^2 \\
&=\norm{Ax^{t+1}-y+w}^2
\leq 2 \norm{Ax^{t+1}-y}^2+ 2\norm{w}^2.
%\norm{y-Ax^{t+1}}^2 &\leq \norm{A(x_0-x^{t+1})+Aw}^2\\
%&\leq 2\norm{A(x_0-x^{t+1})}^2+ 2\norm{Aw}^2
%&\Longrightarrow \norm{y-Ax^{t+1}}^2 \geq 
\end{align*}
The last inequality uses the triangle inequality and the fact that $(a+b)^2\leq 2a^2+2b^2$. 
As a result, we can deduce the following bound for noisy case:
\begin{align}\label{eq:iterbound}
	\norm{x^{t+1}-x_0}^2 \leq 2\left(\frac{1}{\mu\alpha}-1 \right)\norm{x^t-x_0}^2 + \frac{4}{\alpha}\norm{w}^2+ \frac{2}{\mu\alpha}\epsilon_t,
\end{align}

\todo{Note that for noiseless case $y=Ax_0$ it holds that:
\eq{
	\norm{y-Ax^{t+1}}^2= \norm{A(x^{t+1}-x_0)}^2 \geq \alpha\norm{x^{t+1}-x_0}^2,
}
and therefore we can get sharper bound here:
\begin{align}\label{eq:boundnoiseless}
\norm{x^{t+1}-x_0}^2 \leq \left(\frac{1}{\mu\alpha}-1 \right)\norm{x^t-x_0}^2 +  \frac{1}{\mu\alpha}\epsilon_t,
\end{align}}

We apply the previous bound recursively and complete the proof:
\begin{align}
&\norm{x^{t}-x_0}^2 \nonumber \\
&\leq \rho^t  \norm{x^{init}-x_0}^2 +  \frac{4}{\alpha}\norm{w}^2 \sum_{i=0}^{i=t} \rho^i+ \frac{2}{\mu\alpha}\sum_{i=0}^{i=t} \rho^{t-i} \epsilon_i
\end{align}
for $\rho= 2\left(\frac{1}{\mu\alpha}-1 \right)$. Note that for convergence we require $\rho<1$ and therefore a lower bound on the step size which is $1/\mu< 3\alpha/2$.
\end{proof}


{\rem{We achieve a linear convergence (to a solution within $\frac{4(1-\rho^t)}{\alpha(1-\rho)}\norm{w}^2$ distance from $x^0$) as long as $\epsilon_t$ linearly decays to zero:
	\eq{ \norm{x^{t}-x_0}^2 \leq \frac{4(1-\rho^t)}{\alpha(1-\rho)}\norm{e}^2+o( r^t) 
	}	
	\marginpar{shall we say convergence or error decay??} 
	For $\epsilon_t=o(\rho^t)$ we can establish a rate convergence $r=\rho$ similar as for the IPGD algorithm \eqref{eq:IPGD} with the exact projection (see Theorem.2 \cite{Blumen}). 
An approximation with a slower rate of decay, i.e. $\epsilon_t=\Theta(\bar{\rho}^t)$ where $\bar{\rho}<\rho$, decreases the convergence rate of \eqref{eq:eIPGD} to $r=\bar{\rho}$.	
%If decays with a slower rate $\rho'<\rho$, then the rate of convergence of \eqref{eq:eIPGD} will be  
Finally for $\epsilon_t=\Theta(\rho^t)$, we have $r=\rho+ \delta$ for an arbitrary small $\delta>0$.	 	
	}}
	
	
\subsection{Adaptive approximation level}
\todo{Not sure if this part will be useful...didn't work well for MRF simulations}
If we don't know how to set $\epsilon_t$ to decay (probably since we don't know $\rho$), we can for instance do the following adaptive procedure:
\subsubsection{Objective Feedback}
For some constant $0<\gamma<1$ we set the approximation level proportional to the current objective function value:
\eql{\label{eq:adaptive-e}
	\epsilon_t := \gamma \mu  \norm{y-Ax^t}^2.
	}	
% we consider each iteration of \eqref{eq:IPGD} calculates an approximate (inexact) projection step  which obeys the following bound: for solution at each iteration $x^t$ we have
%\eq{
%	\norm{x^t-\Pp_\Mm^\epsilon(x^t)}^2 \leq \norm{x^t-\Pp_\Mm(x^t)}^2 + \epsilon\norm{y-Ax^t}^2
%}	
%We note that the precision of the approximation is not fixed and gradually improved as the objective of \eqref{eq:opt1} decays.
%
%Assume $A$ satisfies Bi-Lipschitz property with respect to $\Mm$ with constants $\alpha,\beta$ defined as follows. 
%
%{\defn{ $A$ is Bi-Lipschitz w.r.t. $\Mm$, if $\forall x1,x2\in \Mm$ there exists constants $0<\alpha\leq \beta$ such that
%	\eql{
%		\alpha \norm{x1+x2}^2 \leq \norm{A(x1+x2)}^2\leq \beta \norm{x1+x2}^2  }	
%}}
The following theorem considers noiseless measurements \marginpar{and it can be extended to noisy measurements case probably with doubling the convergence rate} and states the IPGD convergence using the approximate projection scheme defined above.

{\thm{Assume $y=Ax_0$, and $A$ is Bi-Lipschitz w.r.t. $\Mm$ with constants satisfying $\beta\leq 2\alpha$. Set $0<\gamma<1$ and the step size $\mu>0$ such that
	$\beta \leq 1/\mu \leq (2-\gamma)\alpha$. The sequence generated by Algorithm \eqref{eq:eIPGD} obeys the following bound
	\eql{
		\norm{x^{t}-x_0}^2\leq 
		\left( \frac{1}{\mu\alpha}+\gamma-1\right)^t\norm{x^{init}-x_0}^2.		
	}
}}
\begin{proof}
	Continue from \eqref{eq:boundnoiseless} by substituting $\epsilon_t$ with \eqref{eq:adaptive-e} and then use $\alpha^{-1} \norm{y-Ax^t}^2\leq \norm{x^t-x_0}^2$ 
\end{proof}

\subsubsection{Gradient Feedback}
Norm of the gradient at each iteration can be used for tuning the approximation level i.e. for a positive constant $\gamma$:
\eql{\label{eq:adaptive-e2}
	\epsilon_t := \gamma \norm{g^t}^2 = \gamma\norm{A^*Ax^t-A^*y}^2.
}
	
{\thm{\label{thm:gradconv} Assume $A$ is bi-Lipschitz w.r.t. $\Mm$ with constants $\beta \leq \frac{3\alpha}{2(1+2\gamma\norm{A}^4)}$. Set the step size such that $\frac{2}{3}(1+2\gamma\norm{A}^4)\alpha^{-1}\leq \mu \leq\beta^{-1}$. The sequence generated by Algorithm \eqref{eq:eIPGD} using approximation \eqref{eq:adaptive-e2} obeys the following bound:
			\eql{
			\norm{x^{t}-x_0}^2 
			\leq \rho^t  \norm{x^{init}-x_0}^2  + \frac{4(1-\rho^t)}{\alpha(1-\rho)}\left(1+\gamma \frac{\norm{A}^2}{\mu}\right)\norm{w}^2,
		}
			where, $\rho= 2\left(\frac{1+2\gamma \norm{A}^4}{\mu\alpha}-1 \right)$, 
%\begin{align*}
%&\rho= 2\left(\frac{1+2\gamma \norm{A}^4}{\mu\alpha}-1 \right),\quad\eta=\frac{4(1-\rho^t)}{\alpha(1-\rho)}\left(1+\gamma \frac{\norm{A}^2}{\mu}\right),
%\end{align*}
				 and $w=y-Ax_0$ is the noise.
		}
	}
\begin{proof}
	We have that 
	\begin{align*}
	\gamma\norm{g^t}^2 &= \gamma\norm{A^*A(x^t-x_0)-A^*w}^2\\
	&\leq 2\gamma\norm{A^*A (x^t-x_0)}^2+2\gamma\norm{A^*w}^2\\
	&\leq 2\gamma\norm{A}^4\norm{x^t-x_0}^2+2\gamma\norm{A}^2\norm{w}^2.
	\end{align*}
\marginpar{not sure sharp enough!}The first inequality follows from $(a-b)^2\leq 2a^2+2b^2$. Applying this bound in \eqref{eq:iterbound} we achieve
\begin{align}\label{eq:iterbound2}
\norm{x^{t+1}-x_0}^2 \leq& 2\left(\frac{1+2\gamma \norm{A}^4}{\mu\alpha}-1 \right)\norm{x^t-x_0}^2 \nonumber \\ &+\frac{4}{\alpha}\left(1+\frac{\gamma}{\mu} \norm{A}^2\right)\norm{w}^2.
\end{align}
Applying recursively this bound competes the proof. Note that for convergence we require $\rho<1$ which implies the lower bound on $\mu$.
\end{proof}	

==> sections/manifCS.tex <==
\section{Manifold Compressed sensing}
\label{sec:ManifCS}
\subsection{Exact iterative projected gradient}
Compressed sensing consists of a linear sampling model
\eql{
	\label{eq:CSsampling}
	y \approx Ax_0,
}
where  $y$ is a noisy $m$-dimensional vector of measurements taken from signal $x_0$ in a high dimension $n\gg m$ through using a linear mapping $A$.%and the vector $w$ accounts for bounded noise corruptions.
Variational approach for CS recovery consist in solving following program:
\eql{\label{eq:opt1}
	x^{opt} = \argmin_{x \in \Mm} \norm{y-Ax}_2^2.
}  
First order methods in form of Iterative Projected Gradient (IPG) are very popular to solve \eqref{eq:opt1}. Each iteration has a gradient update followed by a Euclidean projection onto the model $\Mm$ defined as 
\eq{\Pp(x) := \argmin_{u\in\Mm} \norm{u-x}_2^2.}
Starting from the initial point $x^{k=0}=0$, the solution of IPG iteratively updates as follows
\eql{\label{eq:IPGD}
	x^{k+1} = \Pp_{\Mm} \left( x^{k} - \mu A^H(Ax^{k}-y) \right) 
}
until it convergences. % \rightarrow \hat{x} $.	
A general convergence result holds for both convex and non-convex constraints $\Mm$, that is by choosing the step size small enough $\gamma\leq 1/\norm{A}$, IPG converges to a critical point of the problem \eqref{eq:opt1} which for convex $\Mm$ is also a global convergence i.e., $\lim{x^{k}}\rightarrow x^{opt}$.  \nref ATOUCH. 


Remarkably a different line of result guarantees that IPG can globally solve \eqref{eq:opt1} even for the non-convex $\Mm$ constraints. The key assumptions here are the following embedding property and a related properly chosen lower bound on the step size $\mu$.
{\defn{\label{def:bilip} $A$ is Bi-Lipschitz w.r.t. $\Mm$, if $\forall x,x'\in \Mm$ there exists constants $0<\alpha\leq \beta$ such that
		\eql{\label{eq:bilip}
			\alpha \norm{x-x'}^2 \leq \norm{A(x-x')}^2\leq \beta \norm{x-x'}^2  }	
}}
{\thm{\label{th:exactIPG}
[Blumensath'11] Assume $A$ is bi-Lipschitz w.r.t. $\Mm$ and $\xgt\in \Mm$ with constants satisfying $\MM < 1.5\mmx$. Set the step size $2/3\mmx^{-1}<\mu\leq\MM^{-1}$. The sequence generated by IPG Algorithm \eqref{eq:IPGD} obeys the following bound:
		\eql{\label{eq:errbound}
			\norm{x^{k}-\xgt}\leq  \rho^k \norm{\xgt} + \frac{2\sqrt{\MM}}{\mmx(1-\rho)}w
		}
		where,  	
		$\rho=\sqrt{\frac{1}{\mu \mmx} -1}$ 
and $w=\norm{y-A\xgt}$.
}}
\subsection{Iterative approximate projected gradient}
For computational reasons one sometimes requires to consider an approximate model projection. This particularly applies to very complex models where the exact projection is not explicit and amounts to solving an auxiliary optimization at each iteration (or for instance conducting an expensive exhaustive search as will be later discussed in the MRF application). Fortunately the IPG algorithm is shown to be robust against approximations. We define below a widely applicable notion of near-optimal approximation for the projection step:

{\defn{ The $(1+\epsilon)$-approximate projection is defined as follows and for a given $\epsilon\geq0$:
\eql{\label{eq:eproj}
	\pp_\Mm^{\epsilon}(x) \in \Big\{ u\in \Cc :\,	\norm{u-x} \leq (1+\epsilon)\norm{\pp_\Cc(x)-x}  \Big\}. 
}
We note that $\pp_\Mm^{\epsilon}(x)$ might not be unique.}}

 In this regard, the inexact IPG algorithm with a $(1+\epsilon)$-approximate projection takes the following form:
\eql{\label{eq:inIP2}
	x^k = \pp_\Mm^{\epsilon}\left(x^{k-1}-\mu A^H(Ax^{k}-y) \right).}
The following result states that if the embedding holds (with a better conditioning compared to the exact IPG case) then the inexact algorithm  still achievs the accuracy of the exact IPG.

{\thm{\label{th:inexactLS2} Assume $A$ is bi-Lipschitz w.r.t. $\Mm$ and $\xgt\in \Mm$ and that
\eq{\sqrt{\epsilon+\epsilon^2}\leq \delta\frac{\sqrt{\mmx}}{\vertiii{A}} \qandq \MM < (2-2\delta+\delta^2) \mmx} 	
for $\epsilon\geq 0$ and some constant $\delta \in [0,1)$.
		Set the step size $\left((2-2\delta+\delta^2) \mmx\right)^{-1}<\mu\leq\MM^{-1}$. The sequence generated by Algorithm \eqref{eq:inIP2} obeys the following bound:
		\eq{
			\norm{x^{k}-\xgt}\leq  \rho^k \norm{\xgt} + 
			%\frac{ \left( 2\frac{\sqrt{M}}{m}+\frac{\sqrt\mu}{\norm{A}}\delta \right)}
			\frac{\kappa_w}{1-\rho}w
		}
		where 
		\begin{align*}
		\rho=\sqrt{\frac{1}{\mu \mmx} -1}+ \delta, \quad
		\kappa_w= 2\frac{\sqrt{\MM}}{\mmx}+\sqrt\mu\delta, \quad
		 w=\norm{y-A \xgt}.
		\end{align*}		
		
	}} 	
	{\rem{Increasing $\epsilon$ limits the recovery guaranty and slows down the convergence (by comparing $\rho$ in Theorems 1 and 2).}}


\subsection{Manifold embedding results}
The embedding holds when $A$ drawn at random from certain distributions (e.g. element-wise i.i.d. subgaussian, or random row selection of orthonormal bases) and when number of the measurements $m \approx O(\dim(\Mm))$. 

{\thm{[Wakin, Baraniuk'09] Let $\Mm\in \RR^n$ be a compact Riemannian manifold with dimension $\dim(\Mm)$, condition number $1/\tau$, volume $V$ and Geodesic regularity $R$. Then a random orthoprojector $A\in\RR^{m\times n}$ with probability $1-\xi$ provides a bi-Lipschitz embedding on $\Mm$ with $\mmx=1-\theta, \MM=1+\theta$, given 
\eql{
	m=O\Big(\dim(\Mm)\log(nVR\tau^{-1})\theta^{-2}\log(\xi^{-1})\Big)
	}		
for positive constants $\xi,\theta<1$.
}}
		
Embeddable manifolds:
\begin{itemize}
	\item Smooth manifolds with bounded condition number $1/\tau$ \nref[Richwakin][Clarkson]
	\item Doubling sets with finite resolution $\forall x,x'\in \Mm \norm{x-x'}>\Delta_{\min}$ \nref[Indyk'08].
	\item Smooth manifolds are doubling\nref[Dasgupta'12].   
\end{itemize}
%\todo{Results for manifold IPGD, with that perhaps others can be more summerized} 
\subsection{Discretization}\label{sec:discrete}
In this part we consider compressed sensing of signals living on a compact \emph{discrete} manifold $\Mb$ with low intrinsic dimension. The set $\Mb$ may be a dense collection of samples from a continuous manifold with a non trivial projection.
% As the projection step might not be trivial or computationally easy for many complex manifolds we consider a data driven approach which consists of collecting discrete samples of the manifold in a dictionary and approximate 
With such formalism the projection step reduces to searching the nearest atom, however (potentially) in a very large dictionary. 
%With such formalism, the size of discrete manifold $\Mb$ may very large, bringing both storage and computational concerns to the nearest matching step.
This is also related to the \emph{Data driven} compressed sensing framework (with applications in e.g. Hypercritical imagery \cite{TIPHSI}, Mass spectroscopy \nref, MALDI imaging \cite{Kobarg2014}) where in absence of an algebraic physical model one resorts in collecting a large number of data samples in a dictionary and use it as a \emph{point cloud} model for CS reconstruction~\cite{RichCSreview}.  

%In this case the model is $\Mm = \bigcup_{i=1}^{d}\{\psi_i\}$ where $\psi_i\in\RR^n$s are atoms of a $n\times d$ dictionary $\Psi$. %\{\psi_i\}_{i=1}^{d}$
% of $d$ points (atoms) in $\RR^n$ the model becomes.  
%Data driven CS finds numerous applications e.g. in Hypercritical imagery \cite{TIPHSI}, Mass spectroscopy \nref, MALDI imaging \cite{Kobarg2014} and Magnetic Resonance Fingerprinting (MRF)~\cite{MRF,BLIPsiam} just to name a few\todo{add more}. For instance the USGS Hyperspectral library \footnote{\url{http://speclab.cr.usgs.gov}} contains the spectral signatures (reflectances) of hundreds of substances measured across $\sim 400$ frequency bands. This side information is shown to be useful for CS reconstruction and classification in both convex and nonconvex settings (see e.g. \cite{TIPHSI} for more details and its relations to sparse approximation in redundant dictionaries).  
%Recently MR Fingerprinting~\cite{MRF} proposed a fast CS acquisition scheme for quantifying the NMR properties (such as the $T1,T2$ relaxation times, off-resonance frequencies, proton density) of tissues. Since random excitation sequences generate magnetization responses in non-analytic forms, \cite{MRF} proposed build a very large dictionary of fingerprints driven by the Bloch dynamic equations for all combination of those parameters. 

Data driven CS may also apply to algebraic models with non trivial projections. For example in the MR Fingerprinting problem one first constructs a dictionary of magnetization responses (across the readout times) for many $T1,T2$ relaxation values presented in normal tissues \cite{MRF}. This corresponds to sampling a two-dimensional manifold associated with the solutions of the \emph{Bloch dynamic  equations}, which in the MRF settings neither the response nor the projection has a analytic closed-form solution. In this setting the discrete model reads
\eql{\label{eq:discrete}
	\Mb:=\bigcup_{i=1}^{d}\{\psi_i\} \in \RR^J}
that is a point cloud model associated with atoms of a dictionary $\Psi$ customized for e.g. HSI, MALDI or MRF data.

In a single dimensional setting 
i.e. when $x$ is a vector in $\RR^n$  there will be no need for an IPG algorithm to solve problem \eqref{eq:opt1} for a discrete model $\Mm=\Mb$. In fact if the embedding i.e. Definition~\ref{def:bilip} holds with a $\mmx>0$, then a \emph{single step} nearest neighbour matching can solve the problem with a noise robustness depending on the constant $\mmx$.


%the set $\Mm$ may also be a dense collection of samples from a continuous algebraic manifold with a non trivial projection e.g. Magnetic resonance fingerprinting \nref. 
% As the projection step might not be trivial or computationally easy for many complex manifolds we consider a data driven approach which consists of collecting discrete samples of the manifold in a dictionary and approximate 




%Recently MR Fingerprinting \cite{MRF} proposed a fast CS acquisition scheme for quantifying the NMR properties (namely the $T1,T2$ relaxation times) of tissues. Small number of  excitations in form of rotating the magnetic field applies to the tissue, and between each two excitations, the \emph{partial} k-space information is measured. An iterative exact projection algorithm (BLIP) is proposed for the MRF problem which achieves a great parameter estimation accuracy \cite{BLIPsiam}. % versus compression trade-off $\nref$.
%The projection consists of NN searches on a densely sampled manifold $\Mb$ of fingerprints driven by the Bloch dynamic equations.


